Optimal Efficiency-Envy Trade-Off via Optimal Transport

We consider the problem of allocating a distribution of items to $n$ recipients where each recipient has to be allocated a fixed, prespecified fraction of all items, while ensuring that each recipient does not experience too much envy. We show that this problem can be formulated as a variant of the semi-discrete optimal transport (OT) problem, whose solution structure in this case has a concise representation and a simple geometric interpretation. Unlike existing literature that treats envy-freeness as a hard constraint, our formulation allows us to \emph{optimally} trade off efficiency and envy continuously. Additionally, we study the statistical properties of the space of our OT based allocation policies by showing a polynomial bound on the number of samples needed to approximate the optimal solution from samples. Our approach is suitable for large-scale fair allocation problems such as the blood donation matching problem, and we show numerically that it performs well on a prior realistic data simulator.

==> ComputingTheSolution.tex <==
Theorem~\ref{thm:optimal partition} shows that Algorithm~\ref{algo: Normal
Partition Matching} is an elegant optimal solution to the resource allocation
with distributional target constraints in \eqref{prob: optimal partition problem}.
However, it is a-priori unclear whether Step 1 of Algorithm~\ref{algo: Normal
Partition Matching} can be efficiently computed. The goal of the next two
sections is to resolve this question positively.

We will start by assuming access to an oracle function $\oraclep(\cdot)$ which takes as input a shift vector $v$ (and
implicitly, a distribution $\cD$), and outputs the resulting matching
probabilities for each recipient, $\oraclep(v) \in \Delta^n$. 
Our goal will then be to find a shift vector $v$ such that
its' matching distribution $\oraclep(v)$ is close to the target matching
distribution $\optp$.  We use the the $L1$ norm to measure this distance:
\begin{equation}
    L(v) = ||\oraclep(v)-\optp||_1
    \label{eq: minimizing square loss}
\end{equation}
% \todo{but Lemma 2 is not proven yet? And it's supposedly based on the algorithm; it's a bit iffy to refer to it here I think}
% Lemma~\ref{lem:unique normal partition} implies that there exists optimal
% solution $v^*$ such that $L(v^*) = 0$. 
Before we discuss the algorithm for minimizing $L(\cdot)$, one might wonder how this
new objective relates to the original objective $f(\cdot)$ as defined in
\eqref{prob: optimal partition problem}. Intuitively, since Lemma~\ref{lem:
normal partition is optimal} shows that any normal partition is optimal among all
other partitions that have the same matching distribution, an approximate
solution to \eqref{eq: minimizing square loss} should give us an approximate
solution to \eqref{prob: optimal partition problem} as well.  The next lemma
shows that this is indeed the case.  Let $\OPT$ be the optimal value of
\eqref{prob: optimal partition problem}. 
\begin{proposition}
    Suppose we are given a normal partition $\{\Omega_i\}$ characterized by shift
    vector $v$ such that $L(v)\leq \epsilon$. Then $\OPT - f(\{\Omega_i\})\leq
    \epsilon n\bar x$, and $|\oraclep(v)_i-\optp_i|\leq \epsilon \,\forall i$.
    \label{prop: new formulation approximately solves the original}
\end{proposition}
The proof of Proposition~\ref{prop: new formulation approximately solves the original}
can be found in Section~\ref{sec: auxiliary proofs}.  We now present
Algorithm~\ref{algo: LineSearch Normal Partition Matching}, which is designed to
solve \eqref{eq: minimizing square loss} efficiently.
% As mentioned earlier, shifting all entries in the shift vector by a constant
% does not change the normal partition. Therefore, we can always modify the shift
% vector so that the minimum entry is equal to zero without changing the matching
% distribution or the utlities associated with the normal partition.
\begin{algorithm}
    \DontPrintSemicolon % Some LaTeX compilers require you to use \dontprintsemicolon instead
    \KwIn{Distribution $\cD$, and target matching distribution $p$. Initial shift vector $v=[0,\ldots,0]$.}
    \For{$t \gets 0, 1, 2, \ldots$} {
    
      \If{$L(v) \leq \epsilon$} {
        \Return $v$\;
      }
      $i^* \gets \argmin\limits_{i\in[n]} \oraclep(v)_i - \optp_i$\; \label{step: find min recipient}
      Increase $v_{i^*}$ until $\oraclep(v)_i = \optp_i$\; \label{step: line search}
    }
    \caption{LineSearch Normal Partition Matching}
    \label{algo: LineSearch Normal Partition Matching}
\end{algorithm}
Step~\ref{step: line search} in the algorithm could be done using line search,
hence the name of the algorithm. We show that the number of iterations for this
algorithm to terminate is bounded:
\begin{theorem}
    Algorithm~\ref{algo: LineSearch Normal Partition Matching} terminates after
    at most $4\frac{n^3\bar x\bar \mu}{\epsilon}$ iterations.
    \label{thm: polynomial time algorithm}
\end{theorem}

\subsection{Proof of Lemma~\ref{lem:unique normal partition} and Theorem~\ref{thm:
polynomial time algorithm}}
\begin{proof}
\textbf{Existence:} 
% Let $\oraclep(v)$ represent the vector in $\bbR^n$ where each entry represents the
% total probability mass matched to each of the recipients under the shift vector
% $v$.  
Let $I(v)$ represent the set of recipients who are \emph{over matched}
under the normal partition characterized by shift vector $v$: $I(v)
\coloneqq\{i: \oraclep(v)_i > \optp_i\}$.  Let $\Delta(v)$ be a potential
function that represents the total amount of over-matched probability mass:
$\Delta(v) = \sum_{i\in I(v)} \oraclep(v)_i - \optp_i$.  The idea of the proof is as follows: If we can show that Algorithm~\ref{algo: LineSearch Normal Partition
Matching} generates a sequence of bounded shift vectors such that $\Delta(v_t)$
converges to $0$, then by the Bolzano-Weierstrass theorem there exists a shift
vector $v$ such that $\Delta(v)=0$, which means that $\oraclep(v)$ 
matches the target matching distribution.
We use $I_t$ to denote $I(v_t)$ and $\Delta_t$ to denote $\Delta(v_t)$. 
% First, note that by Assumption~\ref{assumption: regularity of the distribution},
% we know that if a normal partition exists, then it can be represented by a shift
% vector $v$ such that $v_i \in [0,\bar x]$. This is because 1) adding a constant
% to the shift vector does not change the normal partition, and 2) the difference
% between any two entries in the shift vector should not exceed $\bar x$. To see
% the second point, suppose $v_i - v_j > \bar x$, then $X_i + v_i > X_j + v_j$
% with probability $1$, which means that $j$ will be matched with probability $0$,
% a contradiction.

% When
% there is no ambiguity, we drop the time index $t$ and use $v$ to represent the
% ``current'' shift vector.  We also use $\oraclep$ instead of $\oraclep(v)$ to
% denote the matching distribution given by the current shift vector. 
% If they are the same as the target matching
% probability then we are done. Otherwise, consider the set of recipients who are
% initially matched too often: $$\cI = \{i: \tilde p_i>p_i\}$$ Let $\Delta$ be the
% total amount of probability by which recipients $\cI$ are receiving too much of:
% $$\Delta = \sum_{i\in\cI} \max\{ \tilde p_i - p_i, 0\}$$
% 
% In each round, we find the recipient who is currently receiving the fewest
% matches relative to their target probability i.e., $ i =\argmin_j \tilde p_j -
% p_j$, and shift $v_i$ down (which increases the chances of matching $i$) until
% $\tilde p_i = p_i$.
% 
When we increase the shift value for recipient $i^*$ in Step~\ref{step: line
search}, the matching probabilities for other recipients can only decrease, so
this procedure will never increase $\Delta_t$, and it will never push any
recipient $i\not\in I_t$ into receiving too much. This means that the set of
over-matched recipients can only decrease: $I_0\supseteq I_1\supseteq I_2
\ldots$. This has a couple of implications:
\begin{enumerate}
    \item For any $t$, there exists $i$ such that $v_{ti} = 0$.
    \item $v_{ti} \in [0, \bar x]$ for all $t$, $i$.
    % \item $\Delta_t$ is monotonically decreasing.
\end{enumerate}
The first one follows from the fact that the algorithm only increases the shift
value for $i\notin I$. So either $I$ is never empty, in which case the shift
values for those remaining in $I$ are always $0$. Or, $I$ becomes empty at some
point, in which case the last recipient to leave $I$ has a shift value of $0$.
To see the second point, suppose $v_{ti}>\bar x$ for some $t, i$. Clearly
$i\notin I_t$. Now if $I_t\neq \emptyset$, then $p(v_t)_j = 0$ for all $j\in
I_t$. This is because $\bbP(X_j > X_i+v_{ti}) = 0$ for all $j\in I_t$. But this
contradicts these recipients being over matched.  On the other hand, if $I_t$ is
empty, that means a perfect solution is found.  But by the same reasoning,
$p(v_t)_j = 0$, where $j$ is the last recipient who left $I$.  This contradicts
our assumption that $\optp_j>0$. This second observation will come in handy later
in the proof. For now, we note that since $\Delta_t$ is non-increasing, it has
to converge to either $0$ or a positive number.



% The proof completes if we can show that $\lim\limits_{t\rightarrow
% \infty}\Delta_t \rightarrow 0$ through this procedure (and that $v$ lie in some
% kind of compact set).

Suppose for contradiction that $\lim\limits_{t\rightarrow \infty}\Delta_t
\rightarrow \Delta' >0$.  This means that $I_t$ is never empty. 
% Secondly, this means that $v_{ti} \in [0, \bar x] $ for all $i$ and all times
% $t$.  To see this, first note that since the shift vectors are initialized to
% zero and $I_t$ is a decreasing sequence, we know that $v_{ti} = 0$ for all $t$
% and $i\in I_t$.  Now if at some timestep $t$, $v_{tj} > \bar x$ for some
% $j\notin I_t$, then $\bbP\left(X_i+v_i \geq X_j + v_j\right) = 0$ for all $i\in
% I_t$, which means $\oraclep_i(v_t) = 0$ for all $i\in I_t$. This contradicts
% $I_t$ being the set of overmatched recipients, so $v_{ti} \in [0, \bar x] $ for
% all $i$ and all times $t$. 
% Now, we show that it cannot be the case that $v_i \in [0, \bar x] \,\forall i$
% at all times, which would prove that $\lim\limits_{t\rightarrow \infty}\Delta_t
% = 0$ by contradiction.
% Now, under our assumption $\lim\limits_{t\rightarrow \infty}\Delta_t \rightarrow
% \Delta' >0$ we have that $I_t$ is decreasing and never empty, and therefore 
Combined with the fact that $I_t$ is decreasing, this means that we can find a
recipient $i$ who is always over allocated.  
By the pigeonhole principle, the recipient chosen in Step~\ref{step: find min
recipient} in every round must satisfy $ \oraclep(v_t)_{i^*} - \optp_{i^*} \leq
-\frac{\Delta'}{n}$.  In order for this recipient to get the correct matching
probability, we need to increase $v_{i^*}$ by at least $\frac{\Delta'}{n^2
\bar\mu}$ (by Assumption~\ref{assumption: regularity of the distribution}).  The
extra factor of $1/n$ comes from the fact that as we increase $v_{i^*}$ we are
taking probability masses away from $n-1$
other recipients. Since this is a quantity that does not decrease with time, as
the algorithm continues, there must be at least one entry in the shift vector
that goes to infinity. This contradicts the $v_i \in [0, \bar x] \,\forall i$
result we derived above.
So, by contradiction, $\Delta_t\rightarrow 0$. 


\textbf{Uniqueness:}
    Uniqueness (up to differences with measure zero) directly follows from
    Lemma~\ref{lem: normal partition is optimal}. 

    
\textbf{Polynomial number of iterations (Theorem~\ref{thm: polynomial time
algorithm}):} We showed above that the algorithm has to terminate. Now we show
that it has to terminate within $\frac{4n^3\bar x\bar \mu}{\epsilon}$
iterations. 

Given an initial shift vector, let $\Delta_0$ be the corresponding initial
mismatched probability.  As long as $\Delta_t > \frac12 \Delta_0$, we know that
the shift vector for some $j\notin I $ increases by at least
$\frac{1}{2}\frac{\Delta_0}{n^2 \bar \mu}$.  
% \todo{I agree this was shown above, but it's kind of hidden because the
% structure makes it look like it's dependent on the "suppose for contradiction"
% part. Could you restructure the proof slightly to make it a separate thing?}
Since we know that shift vector never
exceeds $\bar x$, the potential function can stay above $\frac{\Delta_0}{2}$ for
at most $\frac{\bar x n}{\frac{1}{2}\frac{\Delta_0}{n^2\bar \mu}} = 2\frac{n^3
\bar x\bar \mu}{\Delta_0}$ iterations. 
After that, the potential function can stay above $\frac{\Delta_0}{4}$ for at most 
$4\frac{n^3
\bar x\bar \mu}{\Delta_0}$ additional iterations. Repeating this process, we
conclude that the total number of iterations it takes
before $\Delta$ has to drop below $\frac{1}{2}\epsilon$ is then bounded by 
% \todo{could you add a bit mroe detail to this argument?}
$$2\frac{n^3 \bar x\bar \mu}{\epsilon}
+ 2\frac{n^3 \bar x\bar \mu}{2\epsilon} 
% 2\frac{n^3 \bar x\bar \mu}{4\sqrt{\epsilon}} 
+ \ldots + 2\frac{n^3 \bar x\bar \mu}{\Delta_0} \leq 4\frac{n^3
\bar x\bar \mu}{\epsilon}$$
The proof finishes by noting that $$L(v) = ||\oraclep - \optp||_1 =
2\Delta \leq \epsilon.$$



\end{proof}



\section{Relaxing the Oracle Assumption}
\label{sec: weaker oracle}
The line search step (Step~\ref{step: line search}) in Algorithm~\ref{algo:
LineSearch Normal Partition Matching} could potentially be expensive, since it
may involve many calls to the matching distribution oracle, which itself can be
expensive in practice. 
In this section, we design a different algorithm whose step size can be more
easily determined, rather than having to resort to using a line search oracle.
Since normal partitions are characterized by a shift vector, there is a natural
approach for iteratively adjusting the shift vector $v$:
\begin{itemize}
    \item In every round, calculate the matching distributions
    given the current shift vector $v$.
    \item Decrease the shift vector for recipient $i$ if it is receiving more
    than the target matching distribution ($\oraclep(v)_i>\optp_i$), and vice-versa.
\end{itemize}

The question is then whether such an updating scheme is guaranteed to converge to a solution,
potentially under some conditions on the step sizes used in the adjustments.
We show that this is indeed the case. 
The key lemma for our
next algorithm is to show that $p(v)_i-p^*$ acts as a descent direction.
To show this, we  let $v^*$ be a shift vector that has the target
matching distribution; we remind the reader that there can potentially
be multiple shift vectors that are optimal (e.g.  when there is zero probability
mass around the boundaries), so $v^*$ need not be unique. 
\begin{lemma}
    % For $v$ such that $||\tilde p(v) - p||_1 > \epsilon$, 
    $\sum\limits_{i=1}^n (v_i-v^*_i)(\oraclep(v)_i - \optp_i) \geq
    \frac{||\oraclep(v)-\optp||_1^2}{2n\bar\mu}$
    \label{lem: descent direction}
\end{lemma}
\begin{proof}
    Let the partition corresponding to the current shift vector $v$ and the
    optimal shift vector $v^*$ be $\{\Omega_i\}$ and $\{\Omega_i^*\}$ respectively.
    WLOG, we sort the recipient indices in the decreasing order of $v_i-v^*_i$
    (i.e., $v_1-v^*_1 \geq v_2 - v^*_2 \geq \ldots$). 
    % In the following
    % calculations, we use $p_i$ instead of $p(v)_i$ to denote the current
    % matching distribution given $v$.

    Let $q_{ij} = \bbP( \Omega_i \cap \Omega_j^*)$ be the ``error flow'' from
    $j$ to $i$. Note that since we ordered the recipients in decreasing order of
    $v_i-v^*_i$, we have that $q_{ij} = 0$ for $i>j$. This is because if
    $X_j+v^*_j > X_i+v^*_i$ then $X_j + v_j > X_i + v_i$.  We immediately have
    the following two relationships:
    \begin{equation}
        \oraclep(v)_i - \optp_i = \sum_{i<j} q_{ij} - \sum_{j<i}q_{ji}
        \label{eq: matching difference decomposition}
    \end{equation}
    \begin{equation}
        \sum\limits_{i=1}^n (v_i-v^*_i)(\oraclep(v)_i - \optp_i) = \sum_{i<j} q_{ij} \left[(v_i - v^*_i) - (v_j - v^*_j)\right]
        \label{eq: improvement decomposition}
    \end{equation}

    First note that for any $i<j$:
    $q_{ij} \leq \bbP(X_j + v^*_j > X_i + v^*_i) - \bbP(X_j+v_j > X_i + v_i)
    \leq \bar\mu (v_i-v_j - (v_i^*-v_j^*))$,
    where the last inequality follows from Assumption~\ref{assumption: regularity of the distribution}.
    Therefore $(v_i -
    v^*_i) - (v_j - v^*_j) \geq \frac{q_{ij}}{\bar \mu}$. 
    Additionally, it follows from \eqref{eq: matching difference decomposition}
    that $||\oraclep(v) - \optp||_1 \leq \sum_i \left(\left|\sum_{j>i} q_{ij}\right| +
    \left|\sum_{j<i} q_{ji}\right| \right)\leq  2||q||_1$. Using these
    results, we have
    \begin{align*}
    \sum\limits_{i=1}^n (v_i-v^*_i)(\oraclep(v)_i - \optp_i) = &\sum_{i<j} q_{ij} \left[(v_i - v^*_i) - (v_j - v^*_j)\right]\\
    \geq & \sum_{i<j} \frac{q_{ij}^2}{\bar \mu}\\
    \geq & \frac{||q||_1^2}{n\bar \mu}\\
    \geq & \frac{||\oraclep(v)-\optp||_1^2}{2n\bar \mu}
    \end{align*}
    where in the second to last inequality we used the fact that $||q||_2\geq
    ||q||_1/\sqrt{n}$.


    % $$\sum_{i<j} \frac{q_{ij}^2}{\bar \mu} \geq \frac{\epsilon^2}{n\bar \mu}$$

    % Then for $j+1$:
    % \begin{align*}
    %     &\sum\limits_{i=1}^{j+1} (p_i-p^*_i)(v_i - v^*_i)\\
    %     \geq & (v_j-v^*_j) \sum\limits_{i=1}^j (p_i-p^*_i)  + (v_{j+1} -
    %     v^*_{j+1})(p_{j+1}-p^*_{j+1})\\
    %     \geq & (v_{j+1}-v^*_{j+1}) \sum\limits_{i=1}^j (p_i-p^*_i)  + (v_{j+1} -
    %     v^*_{j+1})(p_{j+1}-p^*_{j+1})\\
    %     = & (v_{j+1}-v^*_{j+1})\sum\limits_{i=1}^{j+1} (p_i-p^*_i)  
    % \end{align*}
\end{proof}
Lemma~\ref{lem: descent direction} shows that given $v$, $-(\oraclep(v) - \optp)$ is always
a descent direction, even though the gradient $\nabla L(v)$
is not necessarily in the same direction as $\oraclep(v)-\optp$. 
% This observation might be of independent interest in other optimization problems
% where this kind of property holds.
Armed with Lemma~\ref{lem: descent direction}, we design a new algorithm for
finding the optimal shift vector by moving in the direction of
$-\oraclep(v)+\optp$ in each step. 
The new algorithm is presented in
Algorithm~\ref{algo: Constant Stepsize Normal Partition Matching}.

% Then we can try to mimic the analysis in \cite{hazan2015beyond}.
\begin{algorithm}
    \DontPrintSemicolon % Some LaTeX compilers require you to use \dontprintsemicolon instead
    \KwIn{Distribution $\cD$, and target matching distribution $p$. Initial
    shift vector $v=[0,\ldots,0]$. Learning rate $\eta$.}
    \For{$t \gets 0, 1, 2, \ldots, T$} {
      $v_{t+1} = v_t - \eta (\oraclep(v_t) - \optp)$\;
    }
    \KwRet{$\bar v_T = \argmin_{\{v_1,\ldots, v_T\}} L(v_t)$}\label{step: argmin in constant step algo}
    \caption{Constant Step Size Normal Partition Matching}
    \label{algo: Constant Stepsize Normal Partition Matching}
\end{algorithm}

In typical optimization literature, a zeroth-order optimization method would
only have access to a function evaluation oracle, which is
$L(v) = ||\oraclep(v)-\optp||_1$ in our case. A first-order optimization method would
have access to the gradient oracle, which is $\nabla L(v)$. 
In contrast, we only require oracle access to $\oraclep(v)$, which is in between
a zeroth-order and first-order oracle. This insight might be of independent
interest in other optimization problems. Our main result for this section is the
following bound on the number of iterations it takes for Algorithm~\ref{algo: Constant Stepsize Normal Partition Matching} to find an approximate solution.

\begin{theorem}
    Algorithm~\ref{algo: Constant Stepsize Normal Partition Matching} with step
    size $\eta = \frac{1}{2n\bar\mu}$ finds an
    $\epsilon$ optimal point (i.e., $L(v) \leq \epsilon)$ within $T =
    \frac{4n^3\bar\mu^2||v_0-v^*||^2_2}{\epsilon^2}$ iterations.
    \label{thm: constant step size convergence result}
\end{theorem}
\begin{proof}
    % Assuming that the shift vector $v_t$ is such that $||\tilde p(v_t) -
    % p||_1 \geq \epsilon$ for $t=1,\ldots, T$, then
    We use $\oraclep_t$ to denote $\oraclep(v_t)$.
    \begin{align*}
    &||v_{t+1} - v^*||^2 \\
    (\text{Algebra})=& ||v_t - v^*||^2 - 2\eta \langle v_t-v^*, \oraclep_t - \optp \rangle + \eta^2 ||\oraclep_t - \optp||_2^2\\ 
    (\text{Lemma~\ref{lem: descent direction}})\leq& ||v_t - v^*||^2 - \eta \frac{||\oraclep_t - \optp||_1^2}{n\bar \mu} + \eta^2 ||\oraclep_t - \optp||_2^2\\ 
    (||\cdot||_2 \leq ||\cdot||_1)\leq& ||v_t - v^*||^2 + ||\oraclep_t - \optp||^2_2 \left(- \frac{\eta}{n\bar \mu} + \eta^2\right)\\ 
    (\text{Set $\eta = \frac{1}{2n\bar\mu}$})=& ||v_t - v^*||^2 - \frac{||\oraclep_t - \optp||^2_2}{4n^2\bar\mu^2}
    \end{align*}
    After rearranging and summing over $t=1, \dots, T-1$, we have
    \begin{align*}
        ||v_0 - v^*||^2 - ||v_T-v^*||^2 \geq \sum_{t=1}^{T-1} \frac{||\oraclep_t
        - \optp||_2^2}{4n^2\bar\mu^2}
    \end{align*}
    Suppose $||\oraclep_t - \optp||_1\geq \epsilon$ for $t=1,\ldots, T$, then
    $||\oraclep_t - \optp||_2^2 \geq\frac{\epsilon^2}{n}$ for $t=1,\ldots, T$.
    This means that
    $T \leq \frac{4n^3\bar\mu^2||v_0-v^*||^2_2}{\epsilon^2}$. 

    % \mycomment{
    % If we can further bound $||v_t-v^*|| \leq C ||\tilde p-p||$, then The
    % convergence is $O(n^2\log(\frac{1}{\epsilon}))$}

\end{proof}

Note that Algorithm~\ref{algo: Constant Stepsize Normal Partition Matching} also
gives rise to a natural \emph{stochastic} optimization algorithm, where in each iteration $t$, instead
of using the exact matching distribution $\oraclep(v_t)$ to find the update
direction, we can use a noisy version $\hat p(v_t)$ to perform the updates.
One natural choice for $\hat p_t$ would be $\hat p(v_t) = [\1(i \text{ is matched
under } v_t)]$ for a randomly drawn item $X\sim\cD$.  It is easy to see that
$\bbE[\hat p(v_t)] = \oraclep(v_t)$. 
In convex optimization, first order methods are known to be very robust and
stochastic variations of the same optimization method usually achieve good
guarantees (e.g., stochastic gradient descent vs gradient descent).
However, since the loss function $L(v)$ in our case is not convex with respect
to $v$, it is difficult to get performance guarantee on the average iterate 
$\frac{1}{T}\sum_{t=1}^T v_t$ or the last iterate $v_T$, as typically seen in
convex optimization literature.


==> NeurIPS 22/AuxiliaryProofs.tex <==
% \section{Auxiliary Proofs}
% \label{sec: auxiliary proofs}
% \subsection{Proof of Theorem~\ref{thm: duality of semi-discrete OT}}
% \begin{proof}
% 	Detailed derivation can be found in Section~5.2 of
% 	\cite{peyre2019computational}, as well as Section~7 of
% 	\cite{levy2018notions}.
% \end{proof}

\subsection{Proof of Theorem~\ref{thm: duality of envy constrained OT}}
\begin{proof}
	
Using Fenchel-Rockafellar's duality theorem, the dual of \eqref{eq: individual
envy constraint primal} can be written as 
\begin{align}
    &\max_{f, g, \gamma\geq 0} \int_\cX f(x) d\alpha(x) + g^\top \beta - \sum_{j,k, j\neq k}\gamma_{jk}\lambda_j\label{eq: individual envy constraint dual}\\
    s.t. \quad& \left(1+\sum_{k\neq j} \gamma_{jk}\right)c(x, j) - \sum_{k\neq j}\gamma_{ky}c(x, k)\frac{\beta_k}{\beta_j}\nonumber\\
    & - f(x) - g_j\geq 0 \quad\forall x\in \cX, y_j\in \cY\nonumber
\end{align}

Fixing $g\in \bbR^n$ and $\gamma \in \bbR^{n(n-1)}$, we can check using first
order conditions that the optimal $f(x)$ has the closed form expression:
$$\min\limits_{j\in[n]}\dualg(x, y_j) \coloneqq  \left(1+\sum_{k\neq j}
\gamma_{jk}\right)c(x, j) - \sum_{k\neq j}\gamma_{kj}c(x,
k)\frac{\beta_k}{\beta_j} - g_j$$
Using this, the infinite dimensional optimization problem in \eqref{eq:
individual envy constraint dual} can be transformed to a finite dimensional
optimization problem:
\begin{align}
    \max_{g, \gamma\geq 0}\cE(g,\gamma)\coloneqq\int_\cX  \min_{j\in [n]}\dualg(x, y_j) \,d\alpha(x) + g^\top \beta - \sum_{j,k, j\neq k}\gamma_{jk}\lambda_j\label{eq: individual envy constraint dual finite dim}
\end{align}
Alternatively, we can adapt the Laguerre cell notation in \eqref{eq: optimal
transport dual} to \eqref{eq: individual envy constraint dual finite dim}:
\begin{align}
    \cE(g, \gamma) = \sum_{i\in[n]}\int_{\bbL_{y_i}(g, \gamma)} \dualg(x, y_i)d\alpha(x) + g^\top \beta - \sum_{j,k, j\neq k}\gamma_{jk}\lambda_j\nonumber
\end{align}
where $\bbL_{y_i}(g, \gamma) = \left\{ x\in\cX: y_i = \argmin\limits_{y_j}
\dualg(x, y_j)\right\}$.
\end{proof}

% \subsection{Remaining Proof of Theorem~\ref{thm: sample complexity bound}}
% \begin{proof}
% Continuing from the proof in the main body of the paper.  Let $B = \Fbound$.
% Using Dudley's chaining integral \cite{sridharan,dudley1967sizes}, we have that 
% \begin{align*}
% \Rad_m(F\circ S) \leq& \inf_{\delta'>0} \left\{4\delta' + 12\int_{\delta'}^{B}\sqrt{\frac{\log \cN(\delta, F, ||\cdot||_2)}{m}} d\delta\right\} \\
% (Lemma~\ref{lem: shattering dimension bound} \text{ and }\eqref{eq: covering number bound})\quad
% \leq& \inf_{\delta'>0} \left\{4\delta' + 12\frac{\sqrt{c_1c_0}}{c_2}B\sqrt{\frac{n\log n}{m}}\int_{\delta'}^{B}\sqrt{\log\left(\frac{2B}{\delta}\right)} d\delta\right\} \\
%   = & \inf_{\delta'>0} \left\{4\delta' + 12\frac{\sqrt{c_1c_0}}{c_2}B^2\sqrt{\frac{n\log n}{m}} \frac{2}{3}\left(\log(2B/\delta')^{3/2} + (\log 2)^{3/2}\right)\right\} \\
% (\text{choosing }\delta'=\frac{1}{\sqrt{m}}) = & c'\sqrt{\frac{n\log n (\log m)^3}{m}}
% % O\left(\sqrt{\frac{n\log n\cdot (\log m)^3}{m}}\right)
% \end{align*}

% Plugging the above back to \eqref{eq: uniform bound} and \eqref{eq: uniform
% bound decomposition}, we see that with probability $1-\delta$, 
% $$\cE(g^*, \gamma^*)
% - \cE(\hat g_S, \hat \gamma_S) \leq c'\left(\sqrt{\frac{n\log n (\log m)^3}{m}} + \sqrt{\frac{1\log(1/\delta)}{m}}\right).$$ 
% Conversely, ignoring the log terms, $m$ needs to be at most on
% the order of $\tilde O\left(\frac{n}{\epsilon^2}\right)$ in order for $\cE(g^*, \gamma^*)
% - \cE(\hat g_S, \hat \gamma_S)$ to be bounded by $\epsilon$ with high probability.
% \end{proof}
\subsection{Proof of Theorem~\ref{thm: sample complexity bound}}
\begin{proof}
    We prove the result via uniform convergence:
\begin{align}
    &\cE(g^*,\gamma^*) - \cE(\hat g_S, \hat\gamma_S)\nonumber\\
    =   &\cE(g^*,\gamma^*) - \cE_S(\hat g_S, \hat\gamma_S) + \cE_S(\hat g_S, \hat\gamma_S) - \cE(\hat g_S, \hat\gamma_S)\nonumber\\
    \leq&\cE(g^*,\gamma^*) - \cE_S(g^*,\gamma^*) + \cE_S(\hat g_S, \hat\gamma_S) - \cE(\hat g_S, \hat\gamma_S)\nonumber\\
    \leq&\sup_{g, \gamma}\left(\cE(g, \gamma) - \cE_S(g, \gamma)\right) + \sup_{g, \gamma} \left(\cE_S(g, \gamma) - \cE(g, \gamma)\right)\nonumber\\
    \leq&2\sup_{g, \gamma}|\cE(g, \gamma) - \cE_S(g, \gamma)|\label{eq: uniform bound decomposition}
\end{align}
Clearly, it suffices to show that $\cE_S(\cdot)$ converges uniformly to $\cE(\cdot)$.  
For a given $g, \gamma$, the dual objective
function and its' empirical version can be written as 
$$\cE(g,\gamma) = \bbE_{\alpha}[f(X)], \quad \cE_S(g, \gamma) = \frac{1}{m}\sum_{t=1}^m f(X^t).$$
Then we can rewrite the supremum in \eqref{eq: uniform bound decomposition} as:
\begin{equation}
    \sup_{g, \gamma}|\cE(g, \gamma) - \cE_S(g, \gamma)| = \sup_{f\in F} \left|\bbE_\alpha [f(X)] - \frac{1}{m} \sum_{X\in S} f(X)\right|
\end{equation}

Since $|f(X)|\leq \Fbound$ for all $f\in F, X\in \cX$, it follows from
Theorem~26.5 in \cite{shalev2014understanding} that with probability $1-\delta$,
\begin{align}
    \sup_{f\in F} \bbE_\alpha [f(X)] - \frac{1}{m} \sum_{X\in S} f(X) 
    \leq 2\bbE_{S} \left[\Rad_m(F\circ S)\right] + \Fbound\sqrt{\frac{2\log(2/\delta)}{m}}
    \label{eq: partial uniform bound 1}
\end{align}
and the same also holds by replacing $F$ with $-F$.
% \begin{align}
%     &\sup_{f\in -F} \bbE_\alpha [f(X)] - \frac{1}{m} \sum_{X\in S} f(X) \nonumber\\
%     \leq &2\bbE_{S} \left[\Rad_m(-F\circ S)\right]+ \Fbound\sqrt{\frac{2\log(2/\delta)}{m}}
%     \label{eq: partial uniform bound 2}
% \end{align}
% where 
Here
\begin{equation*}
    \label{eq: Rad definition}
    \Rad_m(F\circ S) \coloneqq \bbE_{\sigma} \left[\frac{1}{m}\sup\limits_f
    \sum_{j=1}^m \sigma_j f(X_j)\right] 
\end{equation*}
is the standard definition of Rademacher complexity of the set $F\circ S$. Since
$\sigma_i$ are $i.i.d.$ Rademacher random variables, it is easy to see that
$\Rad_m(F\circ S) = \Rad_m(-F\circ S)$.
% Since $\sup_{f\in F} \left|\bbE_\alpha [f(X)] - \frac{1}{m} \sum_{X\in S}
% f(X)\right| $ is less than the maximum of the above two supremums (\eqref{eq:
% partial uniform bound 1} and \eqref{eq: partial uniform bound 2}), 
Therefore we
can use a union bound to obtain that with probability $1-\delta$,
\begin{align}
\sup_{f\in F} \left|\bbE_\alpha [f(X)] - \frac{1}{m} \sum_{X\in S} f(X)\right|
\leq2\bbE_{S} \left[\Rad_m(F\circ S)\right] + \Fbound\sqrt{\frac{2\log(4/\delta)}{m}}
\label{eq: uniform bound}
\end{align}

It remains to bound the Rademacher complexity of the $F\circ S$. To do so, we 
use tools from learning theory, and give the following bound on the fat-shattering dimension (\cite{bartlett1996fat}) of the hypothesis class $F$.
\begin{lemma}
    Under Assumption~\ref{assum: boundedness assumptions}, $F$ has
    $\zeta$-fat-shattering dimension of at most
    $\frac{c_0\Fbound^2}{\zeta^2}n\log(n)$, where $c_0$ is some universal constant.
    \label{lem: shattering dimension bound}
\end{lemma}

% \begin{figure}
% \end{figure}

% \begin{figure}[]
% 	\begin{minipage}{0.5\textwidth}
% 	    \centering
% 	    \includegraphics[width=0.5\textwidth]{slanted_dist_tradeoffcurve.png}
% 	    % \label{fig: 2D partition}
% 	\end{minipage}\\
% 	\begin{minipage}{0.5\textwidth}
% 	    \centering
% 	    \includegraphics[width=0.5\textwidth]{slanted_dist_tradeoffcurve.png}
% 	    % \label{fig: 2D augmenting flow}
% 	\end{minipage}
% 	\caption{Left: Artificial data. Right: simulated blood donation data.}
% 	\label{fig: slanted dist trade off curve}
% \end{figure}







% Since $\bbE_S \left[\hat p_S(v)\right] = p(v)$, the remainder the analysis is
% adapted from the standard empirical process theory analysis (see for example
% Chapter 26 and 28 in \cite{shalev2014understanding}). We provide a proof here for completeness.
% We now show that this is indeed the case. The analysis utilizes the now standard
% approach of symmetrization:
% \begin{align*}
%     \sup_v|p(v)_i - \hat p_S(v)_i|
%     =&\sup_v\left|\bbE_{X\sim \alpha}\left[\1\left[ i = \min \left(\argmax_j X[j]+v[j]\right)\right]\right] - \hat p_S(v)_i\right|\\
%     =&\sup_v\left|\bbE_{S'}\left[\hat p_{S'}(v)_i\right] - \hat p_S(v)_i\right|\\

%     \leq&\sup_v\bbE_{S'}\left[\left|\hat p_{S'}(v)_i - \hat p_S(v)_i\right|\right]\\
%     \leq&\bbE_{S'}\left[\sup_v\left|\hat p_{S'}(v)_i - \hat p_S(v)_i\right|\right]
% \end{align*}
% To simplify notaions, let 
% $F = \left\{x\mapsto \1\left[ i = \min \left(\argmax_j
% x[j]+v[j]\right)\right]: v \in \bbR^n\right\}$ be the set of indicator functions
% of whether $i$ is matched given $X$ and a particular shift vector $v$. Taking
% the expectation on both sides of the above equation, and using the
% symmetrization trick, we have 
% \begin{align*}
%     \bbE_S\left[\sup_v|p(v)_i - \hat p_S(v)_i|\right]
%     \leq & \bbE_{S, S', \sigma} \left[\frac{1}{m}\sup\limits_f
%     \left|\sum_{j=1}^m \sigma_j \left(f(X'_j) - f(X_j)\right)\right|\right]\\
%     \leq & 2\bbE_{S, \sigma} \left[\frac{1}{m}\sup\limits_f
%     \left|\sum_{j=1}^m \sigma_j f(X_j)\right|\right]\\
%     \leq & 2\bbE_{S} \left[\Rad_m(F\circ S)\right]
% \end{align*}
% where 
% \begin{equation}
%     \label{eq: Rad abs definition}
%     \Rad_m(F\circ S) \coloneqq \bbE_{\sigma} \left[\frac{1}{m}\sup\limits_f
%     \left|\sum_{j=1}^m \sigma_j f(X_j)\right|\right] 
% \end{equation}
% It remains to bound the Rademacher complexity of the set $F\circ S$. 
% First we show that $F$ has a VC dimension of $n-1$. 

The proof of Lemma~\ref{lem: shattering dimension bound} can be found in the Appendix. The above bound on the fat-shattering dimension can be used to bound the
covering number (see Definition~27.1 of \cite{shalev2014understanding}) of
$F\circ S$.  Theorem~1 from \cite{mendelson2003entropy} states that
\begin{equation}
\cN(\delta, F, ||\cdot||_2)\leq \left(\frac{2B}{\delta}\right)^{c_1 \fat_{c_2\delta}(F)}
\label{eq: covering number bound}
\end{equation}
where $B$ is a uniform bound on the absolute value of any $f\in F$.
% The remainder of the proof uses Dudley integral to
% bound the Rademacher complexity from covering number. 
% Due to space constraints,
% detailed steps are left for the Appendix.
Let $B = \Fbound$, we have that 

\begin{align*}
&\Rad_m(F\circ S)\\
\leq& \inf_{\delta'>0} \left\{4\delta' + 12\int_{\delta'}^{B}\sqrt{\frac{\log \cN(\delta, F, ||\cdot||_2)}{m}} d\delta\right\} \\
\leq& \inf_{\delta'>0} \left\{4\delta' + 12\frac{\sqrt{c_1c_0}}{c_2}B\sqrt{\frac{n\log n}{m}}\int_{\delta'}^{B}\sqrt{\log\left(\frac{2B}{\delta}\right)} d\delta\right\} \\
%   = & \inf_{\delta'>0} \left\{4\delta' + 8\frac{\sqrt{c_1c_0}}{c_2}B^2\sqrt{\frac{n\log n}{m}} \left(\log(\frac{2B}{\delta'})^{\frac{3}{2}} + (\log 2)^{\frac{3}{2}}\right)\right\} \\
 = & c'\sqrt{\frac{n\log n (\log m)^3}{m}}
% O\left(\sqrt{\frac{n\log n\cdot (\log m)^3}{m}}\right)
\end{align*}
Where we used Dudley's chaining integral \cite{sridharan,dudley1967sizes}, 
Lemma~\ref{lem: shattering dimension bound} and \eqref{eq: covering number bound},
and setting  $\delta'=\frac{1}{\sqrt{m}}$ respectively.
Plugging the above back to \eqref{eq: uniform bound} and \eqref{eq: uniform
bound decomposition}, we see that with probability $1-\delta$, 
% $$\cE(g^*, \gamma^*)
% - \cE(\hat g_S, \hat \gamma_S) \leq c'\left(\sqrt{\frac{n\log n (\log m)^3}{m}} + \sqrt{\frac{1\log\frac{1}{\delta}}{m}}\right).$$ 
\begin{equation*}
    \cE(g^*, \gamma^*)
- \cE(\hat g_S, \hat \gamma_S) \leq c'\left(\sqrt{\frac{n\log n (\log m)^3}{m}} + \sqrt{\frac{1\log\frac{1}{\delta}}{m}}\right).
\end{equation*}%
Conversely, ignoring the log terms, $m$ needs to be at most on
the order of $\tilde O\left(\frac{n}{\epsilon^2}\right)$ in order for $\cE(g^*, \gamma^*)
- \cE(\hat g_S, \hat \gamma_S)$ to be bounded by $\epsilon$ with high probability.

% Let $d$ be the VC dimensino of $F$. Let $|F(S)|$ be the number of possible distinct labels on the set $S$ generated
% by the hypotheses in $F$. Then using Massart's lemma and then Sauer's lemma (see for example Lemma~26.8 and Lemma~6.10 in \cite{shalev2014understanding}), we have
% $$\Rad_m(F\circ S) \leq \sqrt{\frac{2\ln (2|F(S)|)}{m}} \leq \sqrt{\frac{2\ln
% \left(2 \sum\limits_{k=0}^d \begin{pmatrix}m\\k\end{pmatrix}\right)}{m}}$$
% \begin{align*}
%     &\Rad_m(F\circ S)\\
%     (\text{Massart's finite lemma}) = &\sqrt{\frac{2\ln (2|F(S)|)}{n}}\\
%     (\text{Sayer's lemma}) =&\sqrt{\frac{2\ln \left(2 \sum\limits_{k=0}^d \begin{pmatrix}m\\k\end{pmatrix}\right)}{n}}
% \end{align*}








% Therefore from \eqref{eq: uniform bound} we obtain that with probability $1-\delta$,
% $$\sup_v|p(v)_i - \hat p_S(v)_i| \leq C\sqrt{\frac{d\log(m)}{m}} + \sqrt{\frac{2\log(4/\delta)}{m}}$$
% for some constant $C$. For $C\sqrt{\frac{d\log(m)}{m}} +
% \sqrt{\frac{2\log(4/\delta)}{m}}$
% to be less than $\epsilon$, we can use standard
% algebraic manipulations to show that it suffices to have 
% $m\geq \frac{2C^2d\log(m)}{\epsilon^2} + \frac{4\log(4/\delta)}{\epsilon^2}$.
% Using the fact that $m\geq 4a\log(2a)+2b \implies m\geq a\log(m)+b$ (see for
% example Lemma~A.2 in \cite{shalev2014understanding}), we know that 
% $$m \geq \frac{8C^2d}{\epsilon^2}\log(4C^2d/\epsilon^2) +
% 8\frac{\log(2/\delta)}{\epsilon^2}$$ is sufficient. This completes the proof for
% the uniform convergence for one recipient. Summing up the estimation error (using
% $\epsilon/n$ instead of $\epsilon$ in the above bound), bounding $d$ with
% Lemma~\ref{lem: shattering dimension bound}, and applying union bound to \eqref{eq: uniform bound
% decomposition} completes the proof of the theorem.

%% This paragraph converts the expectation on Rad to a high probability statement
% To get the high probability bound, we note that $\Rad_m(F\circ S)$ can be viewed
% as a function that takes in $\sigma_1, \ldots, \sigma_m$ as inputs:
% $\phi(\sigma_1, \ldots, \sigma_m) = \Rad_m(F\circ S)$. It's easy to
% see from \eqref{eq: Rad definition} that $|\phi(\sigma_1, \ldots, \sigma_i', \ldots, \sigma_m) -
% \phi(\sigma,\ldots, \sigma_i, \ldots, \sigma_m)| \leq \frac{1}{m}$.


% To get the high probability bound, note that the function $\phi(X_1,
% \ldots, X_m)\coloneqq \sup_v|p(v)_i - \hat p_S(v)_i|$ satisfies the bounded difference property:
% $$|\phi(\sigma_1, \ldots, \sigma_i', \ldots, \sigma_m) -
% \phi(\sigma,\ldots, \sigma_i, \ldots, \sigma_m)| \leq \frac{2}{m}$$
% This is because changing one item $X$ means that we are moving a probability
% mass of $\frac{1}{m}$ from one recipient to another, and this can introduce at
% most $\frac{2}{m}$ difference in the loss function. Therefore, using McDiarmid's
% inequality, we obtain that with probability $1-\delta$, 
% $$\sup_v|p(v)_i - \hat p_S(v)_i| \leq C\sqrt{\frac{d\log(m)}{m}} + \sqrt{\frac{2\ln(2/\delta)}{m}}$$


% For $C\sqrt{\frac{d\log(m)}{m}}$ and $C\sqrt{\frac{d\log(m)}{m}} +
% \sqrt{\frac{2\ln(2/\delta)}{m}}$ to be less than $\epsilon$, we can use standard
% algebraic manipulations to show that we need 
% $$m \geq \frac{4C^2d}{\epsilon^2}\log(C^2d/\epsilon^2) \impliedby m\geq C_1 \frac{d\log(d/\epsilon)}{\epsilon^2}$$ and 
% $$m \geq \frac{16C^2d}{\epsilon^2}\log(16C^2d/\epsilon^2) +
% 16\frac{\log(2/\delta)}{\epsilon^2}\impliedby m\geq C_2 \frac{d\log(d/\epsilon) +
% \log(1/\delta))}{\epsilon^2}$$ respectively.
\end{proof}
Proof of Lemma~\ref{lem: shattering dimension bound}
\begin{proof}
    % Note that for any $f\in F_i$, the function $x\mapsto f(x)$ can be
    % written as $f(x) = w^\top x + b$, where $w_i = -\left(1+\sum_{k\neq i}
    % \gamma_{ik}\right)$, $w_j = \gamma_{ji}\frac{\beta_j}{\beta_i}$, and $b =
    % -g_i$.  
    Theorem~3 in \cite{kontorovich2021fat} shows that $\fat_\zeta(F_{min}) \leq
    \frac{c_0\Fbound^2}{\zeta^2}n\log{n}$.
    Since the shattering dimension is monotone in the size of the set, we are
    done.
    
    % For a given $v$, and an item $X$, $i$ is matched if 
    % $X_i  - X_j \geq v_j - v_i \,\forall j$. Note that this is the intersection
    % of $n-1$ $n$-dimensional halfspaces.
    % It is well known that $n$-dimensinoal halfspaces have a VC dimension of at
    % most $n$. The result then follows from Theorem~1 in \cite{kupavskii2020vc}
    % (and also Theorem~A in \cite{csikos2018optimal}), which says that the VC
    % dimension of the $k$ intersection of sets each with VC dimension $d$ is
    % bounded by $dk\log(k)$.
\end{proof}
\subsection{Experimental Setup}
\label{sec: experimental setup}
For the artificial data, the value utility vectors are generated from $X = [1,
0.7] - Z \begin{bmatrix}0.2, &0\\ 0.8, &0.4\end{bmatrix}$ where $Z\sim Unif(0,
1) \times Unif(0,1)$.  For finding the optimal allocation policy on the
artificial data, we used Algorithm~\ref{algo: Projected SGD for Envy Constrained
Optimal Transport} with $T=2\cdot10^5$. For simulator data, we used $T =
2.5\cdot 10^6$. To generate Figure~\ref{fig: slanted dist allocation plot} we
sampled $6000$ points from the distribution and plotted them, colored by the
allocation. For Figure~\ref{fig: sample complexity plot}, for each $m$ we ran
$16$ trials, sampling a different set of $m$ data points as our training data
per trial. All experiments are run on a 2019, 6-core Macbook Pro laptop. The simulator code is open sourced by \cite{mcelfresh2020matching} at \url{https://github.com/duncanmcelfresh/blood-matching-simulations}, and also included in the supplementary material.


\iffalse







\subsection{Proof of Proposition~\ref{prop: new formulation approximately solves the original}}
\begin{proof}

    The bound on the constraint $|P(\Omega_i) - \optp_i|$ is obvious. We focus
    on the claim on the objective value $f(\{\Omega_i\})$.
    Let the partition corresponding to the current shift vector $v$ and the
    optimal shift vector $v^*$ be $\{\Omega_i\}$ and $\{\Omega_i^*\}$ respectively.
    WLOG, we sort the recipient indices in the decreasing order of $v_i-v^*_i$
    (i.e., $v_1-v^*_1 \geq v_2 - v^*_2 \geq \ldots$). 
    Let $\{p_i\}$ be the current matching distribution given $v$.
    Similarly to the proof of Lemma~\ref{lem: descent direction}, let $q_{ij} =
    \bbP(\Omega_i \cap \Omega_j^*)$ be the error flow from $j$ to $i$.  Note
    that $q_{ij} = 0$ for $i > j$. This is because if $X_j + v^*_j > X_i+v^*_i$,
    then $X_j+v_j > X_i+v_i$. In other words, there is only flow from right to
    left (bigger indices to smaller indices), and not the other way.

    
    First note that each error flow $q_{ij}$ decreases the objective value by at
    most $q_{ij}\bar x$. This is because the worst possible error flow is one
    where we match an item to someone who values it at $0$ instead of
    someone who values it at $\bar x$. Therefore if we can bound $||q||_1$, then
    can bound the gap in the objective function by $||q||_1\bar x$.

    Now let every recipient be represented as a node, and let directed edges
    between the nodes carry weights $q_{ij}$ (i.e., the edge that starts at $j$
    and ends at $i$ carries a flow of $q_{ij}$). Additionally, let each node
    receive an additional input flow of $\optp_i-\oraclep(v)_i$. It is easy to see that
    under such construction, flow conservation is preserved (this is equivalent
    to \eqref{eq: matching difference decomposition}). 
    
    Now we claim that for any ``tail set'' of nodes, e.g., $S_k \coloneqq \{k, k+1,
    \ldots, n\}$, the total outflow (i.e., $\sum_{i\notin S_k, j\in S_k} q_{ij}$)
    from these nodes are equal to $\sum_{j=k}^n \optp_j-\oraclep(v)_j$. To see this, note
    that by the ordering of the indices, there is no flow from $S_k^{\mathsf{c}}$ to $S_k$.
    Therefore, by flow conservation, the total outflow from $S_k$ must be equal
    to the total inflow, which is $\sum_{j=k}^n \optp_j-\oraclep(v)_j$. This holds for any
    $k=1,\ldots, n$.

    Finally, note that the total inflow to any single node $k$ is bounded by the total
    outflow ``from the right'': $\sum_{i\notin S_{k+1}, j\in S_{k+1}} q_{ij}$, plus the
    additional input flow at $k$:
    $\optp_k-\oraclep(v)_k$. Since the total inflow and
    outflow at node $k$ are the same, we can use the finding in
    the above paragraph to conclude that 
    \begin{align*}
    \sum_{j<k} q_{jk}
    \leq &\optp_k-\oraclep(v)_k + \sum_{i\notin S_{k+1}, j\in S_{k+1}} q_{ij}\\
    \leq & \sum_{j=k}^n \optp_j-\oraclep(v)_j 
    \end{align*}

    Therefore $||q||_1 = \sum_{k=2}^n \sum_{j=1}^{k-1} q_{jk} \leq
    \sum_{k=2}^n\sum_{j=k}^n \optp_j-\oraclep(v)_j \leq \sum_{k=2}^n\sum_{j=k}^n
    |\optp_j-\oraclep(v)_j| \leq n ||\optp - \oraclep(v)||_1$.

\end{proof}
\fi

==> NeurIPS 22/ComputingTheSolution.tex <==
Theorem~\ref{thm:optimal partition} shows that Algorithm~\ref{algo: Normal
Partition Matching} is an elegant optimal solution to the resource allocation
with distributional target constraints in \eqref{prob: optimal partition problem}.
However, it is a-priori unclear whether Step 1 of Algorithm~\ref{algo: Normal
Partition Matching} can be efficiently computed. The goal of the next two
sections is to resolve this question positively.

We will start by assuming access to an oracle function $\oraclep(\cdot)$ which takes as input a shift vector $v$ (and
implicitly, a distribution $\cD$), and outputs the resulting matching
probabilities for each recipient, $\oraclep(v) \in \Delta^n$. 
Our goal will then be to find a shift vector $v$ such that
its' matching distribution $\oraclep(v)$ is close to the target matching
distribution $\optp$.  We use the the $L1$ norm to measure this distance:
\begin{equation}
    L(v) = ||\oraclep(v)-\optp||_1
    \label{eq: minimizing square loss}
\end{equation}
% \todo{but Lemma 2 is not proven yet? And it's supposedly based on the algorithm; it's a bit iffy to refer to it here I think}
% Lemma~\ref{lem:unique normal partition} implies that there exists optimal
% solution $v^*$ such that $L(v^*) = 0$. 
Before we discuss the algorithm for minimizing $L(\cdot)$, one might wonder how this
new objective relates to the original objective $f(\cdot)$ as defined in
\eqref{prob: optimal partition problem}. Intuitively, since Lemma~\ref{lem:
normal partition is optimal} shows that any normal partition is optimal among all
other partitions that have the same matching distribution, an approximate
solution to \eqref{eq: minimizing square loss} should give us an approximate
solution to \eqref{prob: optimal partition problem} as well.  The next lemma
shows that this is indeed the case.  Let $\OPT$ be the optimal value of
\eqref{prob: optimal partition problem}. 
\begin{proposition}
    Suppose we are given a normal partition $\{\Omega_i\}$ characterized by shift
    vector $v$ such that $L(v)\leq \epsilon$. Then $\OPT - f(\{\Omega_i\})\leq
    \epsilon n\bar x$, and $|\oraclep(v)_i-\optp_i|\leq \epsilon \,\forall i$.
    \label{prop: new formulation approximately solves the original}
\end{proposition}
The proof of Proposition~\ref{prop: new formulation approximately solves the original}
can be found in Section~\ref{sec: auxiliary proofs}.  We now present
Algorithm~\ref{algo: LineSearch Normal Partition Matching}, which is designed to
solve \eqref{eq: minimizing square loss} efficiently.
% As mentioned earlier, shifting all entries in the shift vector by a constant
% does not change the normal partition. Therefore, we can always modify the shift
% vector so that the minimum entry is equal to zero without changing the matching
% distribution or the utlities associated with the normal partition.
\begin{algorithm}
    \DontPrintSemicolon % Some LaTeX compilers require you to use \dontprintsemicolon instead
    \KwIn{Distribution $\cD$, and target matching distribution $p$. Initial shift vector $v=[0,\ldots,0]$.}
    \For{$t \gets 0, 1, 2, \ldots$} {
    
      \If{$L(v) \leq \epsilon$} {
        \Return $v$\;
      }
      $i^* \gets \argmin\limits_{i\in[n]} \oraclep(v)_i - \optp_i$\; \label{step: find min recipient}
      Increase $v_{i^*}$ until $\oraclep(v)_i = \optp_i$\; \label{step: line search}
    }
    \caption{LineSearch Normal Partition Matching}
    \label{algo: LineSearch Normal Partition Matching}
\end{algorithm}
Step~\ref{step: line search} in the algorithm could be done using line search,
hence the name of the algorithm. We show that the number of iterations for this
algorithm to terminate is bounded:
\begin{theorem}
    Algorithm~\ref{algo: LineSearch Normal Partition Matching} terminates after
    at most $4\frac{n^3\bar x\bar \mu}{\epsilon}$ iterations.
    \label{thm: polynomial time algorithm}
\end{theorem}

\subsection{Proof of Lemma~\ref{lem:unique normal partition} and Theorem~\ref{thm:
polynomial time algorithm}}
\begin{proof}
\textbf{Existence:} 
% Let $\oraclep(v)$ represent the vector in $\bbR^n$ where each entry represents the
% total probability mass matched to each of the recipients under the shift vector
% $v$.  
Let $I(v)$ represent the set of recipients who are \emph{over matched}
under the normal partition characterized by shift vector $v$: $I(v)
\coloneqq\{i: \oraclep(v)_i > \optp_i\}$.  Let $\Delta(v)$ be a potential
function that represents the total amount of over-matched probability mass:
$\Delta(v) = \sum_{i\in I(v)} \oraclep(v)_i - \optp_i$.  The idea of the proof is as follows: If we can show that Algorithm~\ref{algo: LineSearch Normal Partition
Matching} generates a sequence of bounded shift vectors such that $\Delta(v_t)$
converges to $0$, then by the Bolzano-Weierstrass theorem there exists a shift
vector $v$ such that $\Delta(v)=0$, which means that $\oraclep(v)$ 
matches the target matching distribution.
We use $I_t$ to denote $I(v_t)$ and $\Delta_t$ to denote $\Delta(v_t)$. 
% First, note that by Assumption~\ref{assumption: regularity of the distribution},
% we know that if a normal partition exists, then it can be represented by a shift
% vector $v$ such that $v_i \in [0,\bar x]$. This is because 1) adding a constant
% to the shift vector does not change the normal partition, and 2) the difference
% between any two entries in the shift vector should not exceed $\bar x$. To see
% the second point, suppose $v_i - v_j > \bar x$, then $X_i + v_i > X_j + v_j$
% with probability $1$, which means that $j$ will be matched with probability $0$,
% a contradiction.

% When
% there is no ambiguity, we drop the time index $t$ and use $v$ to represent the
% ``current'' shift vector.  We also use $\oraclep$ instead of $\oraclep(v)$ to
% denote the matching distribution given by the current shift vector. 
% If they are the same as the target matching
% probability then we are done. Otherwise, consider the set of recipients who are
% initially matched too often: $$\cI = \{i: \tilde p_i>p_i\}$$ Let $\Delta$ be the
% total amount of probability by which recipients $\cI$ are receiving too much of:
% $$\Delta = \sum_{i\in\cI} \max\{ \tilde p_i - p_i, 0\}$$
% 
% In each round, we find the recipient who is currently receiving the fewest
% matches relative to their target probability i.e., $ i =\argmin_j \tilde p_j -
% p_j$, and shift $v_i$ down (which increases the chances of matching $i$) until
% $\tilde p_i = p_i$.
% 
When we increase the shift value for recipient $i^*$ in Step~\ref{step: line
search}, the matching probabilities for other recipients can only decrease, so
this procedure will never increase $\Delta_t$, and it will never push any
recipient $i\not\in I_t$ into receiving too much. This means that the set of
over-matched recipients can only decrease: $I_0\supseteq I_1\supseteq I_2
\ldots$. This has a couple of implications:
\begin{enumerate}
    \item For any $t$, there exists $i$ such that $v_{ti} = 0$.
    \item $v_{ti} \in [0, \bar x]$ for all $t$, $i$.
    % \item $\Delta_t$ is monotonically decreasing.
\end{enumerate}
The first one follows from the fact that the algorithm only increases the shift
value for $i\notin I$. So either $I$ is never empty, in which case the shift
values for those remaining in $I$ are always $0$. Or, $I$ becomes empty at some
point, in which case the last recipient to leave $I$ has a shift value of $0$.
To see the second point, suppose $v_{ti}>\bar x$ for some $t, i$. Clearly
$i\notin I_t$. Now if $I_t\neq \emptyset$, then $p(v_t)_j = 0$ for all $j\in
I_t$. This is because $\bbP(X_j > X_i+v_{ti}) = 0$ for all $j\in I_t$. But this
contradicts these recipients being over matched.  On the other hand, if $I_t$ is
empty, that means a perfect solution is found.  But by the same reasoning,
$p(v_t)_j = 0$, where $j$ is the last recipient who left $I$.  This contradicts
our assumption that $\optp_j>0$. This second observation will come in handy later
in the proof. For now, we note that since $\Delta_t$ is non-increasing, it has
to converge to either $0$ or a positive number.



% The proof completes if we can show that $\lim\limits_{t\rightarrow
% \infty}\Delta_t \rightarrow 0$ through this procedure (and that $v$ lie in some
% kind of compact set).

Suppose for contradiction that $\lim\limits_{t\rightarrow \infty}\Delta_t
\rightarrow \Delta' >0$.  This means that $I_t$ is never empty. 
% Secondly, this means that $v_{ti} \in [0, \bar x] $ for all $i$ and all times
% $t$.  To see this, first note that since the shift vectors are initialized to
% zero and $I_t$ is a decreasing sequence, we know that $v_{ti} = 0$ for all $t$
% and $i\in I_t$.  Now if at some timestep $t$, $v_{tj} > \bar x$ for some
% $j\notin I_t$, then $\bbP\left(X_i+v_i \geq X_j + v_j\right) = 0$ for all $i\in
% I_t$, which means $\oraclep_i(v_t) = 0$ for all $i\in I_t$. This contradicts
% $I_t$ being the set of overmatched recipients, so $v_{ti} \in [0, \bar x] $ for
% all $i$ and all times $t$. 
% Now, we show that it cannot be the case that $v_i \in [0, \bar x] \,\forall i$
% at all times, which would prove that $\lim\limits_{t\rightarrow \infty}\Delta_t
% = 0$ by contradiction.
% Now, under our assumption $\lim\limits_{t\rightarrow \infty}\Delta_t \rightarrow
% \Delta' >0$ we have that $I_t$ is decreasing and never empty, and therefore 
Combined with the fact that $I_t$ is decreasing, this means that we can find a
recipient $i$ who is always over allocated.  
By the pigeonhole principle, the recipient chosen in Step~\ref{step: find min
recipient} in every round must satisfy $ \oraclep(v_t)_{i^*} - \optp_{i^*} \leq
-\frac{\Delta'}{n}$.  In order for this recipient to get the correct matching
probability, we need to increase $v_{i^*}$ by at least $\frac{\Delta'}{n^2
\bar\mu}$ (by Assumption~\ref{assumption: regularity of the distribution}).  The
extra factor of $1/n$ comes from the fact that as we increase $v_{i^*}$ we are
taking probability masses away from $n-1$
other recipients. Since this is a quantity that does not decrease with time, as
the algorithm continues, there must be at least one entry in the shift vector
that goes to infinity. This contradicts the $v_i \in [0, \bar x] \,\forall i$
result we derived above.
So, by contradiction, $\Delta_t\rightarrow 0$. 


\textbf{Uniqueness:}
    Uniqueness (up to differences with measure zero) directly follows from
    Lemma~\ref{lem: normal partition is optimal}. 

    
\textbf{Polynomial number of iterations (Theorem~\ref{thm: polynomial time
algorithm}):} We showed above that the algorithm has to terminate. Now we show
that it has to terminate within $\frac{4n^3\bar x\bar \mu}{\epsilon}$
iterations. 

Given an initial shift vector, let $\Delta_0$ be the corresponding initial
mismatched probability.  As long as $\Delta_t > \frac12 \Delta_0$, we know that
the shift vector for some $j\notin I $ increases by at least
$\frac{1}{2}\frac{\Delta_0}{n^2 \bar \mu}$.  
% \todo{I agree this was shown above, but it's kind of hidden because the
% structure makes it look like it's dependent on the "suppose for contradiction"
% part. Could you restructure the proof slightly to make it a separate thing?}
Since we know that shift vector never
exceeds $\bar x$, the potential function can stay above $\frac{\Delta_0}{2}$ for
at most $\frac{\bar x n}{\frac{1}{2}\frac{\Delta_0}{n^2\bar \mu}} = 2\frac{n^3
\bar x\bar \mu}{\Delta_0}$ iterations. 
After that, the potential function can stay above $\frac{\Delta_0}{4}$ for at most 
$4\frac{n^3
\bar x\bar \mu}{\Delta_0}$ additional iterations. Repeating this process, we
conclude that the total number of iterations it takes
before $\Delta$ has to drop below $\frac{1}{2}\epsilon$ is then bounded by 
% \todo{could you add a bit mroe detail to this argument?}
$$2\frac{n^3 \bar x\bar \mu}{\epsilon}
+ 2\frac{n^3 \bar x\bar \mu}{2\epsilon} 
% 2\frac{n^3 \bar x\bar \mu}{4\sqrt{\epsilon}} 
+ \ldots + 2\frac{n^3 \bar x\bar \mu}{\Delta_0} \leq 4\frac{n^3
\bar x\bar \mu}{\epsilon}$$
The proof finishes by noting that $$L(v) = ||\oraclep - \optp||_1 =
2\Delta \leq \epsilon.$$



\end{proof}



\section{Relaxing the Oracle Assumption}
\label{sec: weaker oracle}
The line search step (Step~\ref{step: line search}) in Algorithm~\ref{algo:
LineSearch Normal Partition Matching} could potentially be expensive, since it
may involve many calls to the matching distribution oracle, which itself can be
expensive in practice. 
In this section, we design a different algorithm whose step size can be more
easily determined, rather than having to resort to using a line search oracle.
Since normal partitions are characterized by a shift vector, there is a natural
approach for iteratively adjusting the shift vector $v$:
\begin{itemize}
    \item In every round, calculate the matching distributions
    given the current shift vector $v$.
    \item Decrease the shift vector for recipient $i$ if it is receiving more
    than the target matching distribution ($\oraclep(v)_i>\optp_i$), and vice-versa.
\end{itemize}

The question is then whether such an updating scheme is guaranteed to converge to a solution,
potentially under some conditions on the step sizes used in the adjustments.
We show that this is indeed the case. 
The key lemma for our
next algorithm is to show that $p(v)_i-p^*$ acts as a descent direction.
To show this, we  let $v^*$ be a shift vector that has the target
matching distribution; we remind the reader that there can potentially
be multiple shift vectors that are optimal (e.g.  when there is zero probability
mass around the boundaries), so $v^*$ need not be unique. 
\begin{lemma}
    % For $v$ such that $||\tilde p(v) - p||_1 > \epsilon$, 
    $\sum\limits_{i=1}^n (v_i-v^*_i)(\oraclep(v)_i - \optp_i) \geq
    \frac{||\oraclep(v)-\optp||_1^2}{2n\bar\mu}$
    \label{lem: descent direction}
\end{lemma}
\begin{proof}
    Let the partition corresponding to the current shift vector $v$ and the
    optimal shift vector $v^*$ be $\{\Omega_i\}$ and $\{\Omega_i^*\}$ respectively.
    WLOG, we sort the recipient indices in the decreasing order of $v_i-v^*_i$
    (i.e., $v_1-v^*_1 \geq v_2 - v^*_2 \geq \ldots$). 
    % In the following
    % calculations, we use $p_i$ instead of $p(v)_i$ to denote the current
    % matching distribution given $v$.

    Let $q_{ij} = \bbP( \Omega_i \cap \Omega_j^*)$ be the ``error flow'' from
    $j$ to $i$. Note that since we ordered the recipients in decreasing order of
    $v_i-v^*_i$, we have that $q_{ij} = 0$ for $i>j$. This is because if
    $X_j+v^*_j > X_i+v^*_i$ then $X_j + v_j > X_i + v_i$.  We immediately have
    the following two relationships:
    \begin{equation}
        \oraclep(v)_i - \optp_i = \sum_{i<j} q_{ij} - \sum_{j<i}q_{ji}
        \label{eq: matching difference decomposition}
    \end{equation}
    \begin{equation}
        \sum\limits_{i=1}^n (v_i-v^*_i)(\oraclep(v)_i - \optp_i) = \sum_{i<j} q_{ij} \left[(v_i - v^*_i) - (v_j - v^*_j)\right]
        \label{eq: improvement decomposition}
    \end{equation}

    First note that for any $i<j$:
    $q_{ij} \leq \bbP(X_j + v^*_j > X_i + v^*_i) - \bbP(X_j+v_j > X_i + v_i)
    \leq \bar\mu (v_i-v_j - (v_i^*-v_j^*))$,
    where the last inequality follows from Assumption~\ref{assumption: regularity of the distribution}.
    Therefore $(v_i -
    v^*_i) - (v_j - v^*_j) \geq \frac{q_{ij}}{\bar \mu}$. 
    Additionally, it follows from \eqref{eq: matching difference decomposition}
    that $||\oraclep(v) - \optp||_1 \leq \sum_i \left(\left|\sum_{j>i} q_{ij}\right| +
    \left|\sum_{j<i} q_{ji}\right| \right)\leq  2||q||_1$. Using these
    results, we have
    \begin{align*}
    \sum\limits_{i=1}^n (v_i-v^*_i)(\oraclep(v)_i - \optp_i) = &\sum_{i<j} q_{ij} \left[(v_i - v^*_i) - (v_j - v^*_j)\right]\\
    \geq & \sum_{i<j} \frac{q_{ij}^2}{\bar \mu}\\
    \geq & \frac{||q||_1^2}{n\bar \mu}\\
    \geq & \frac{||\oraclep(v)-\optp||_1^2}{2n\bar \mu}
    \end{align*}
    where in the second to last inequality we used the fact that $||q||_2\geq
    ||q||_1/\sqrt{n}$.


    % $$\sum_{i<j} \frac{q_{ij}^2}{\bar \mu} \geq \frac{\epsilon^2}{n\bar \mu}$$

    % Then for $j+1$:
    % \begin{align*}
    %     &\sum\limits_{i=1}^{j+1} (p_i-p^*_i)(v_i - v^*_i)\\
    %     \geq & (v_j-v^*_j) \sum\limits_{i=1}^j (p_i-p^*_i)  + (v_{j+1} -
    %     v^*_{j+1})(p_{j+1}-p^*_{j+1})\\
    %     \geq & (v_{j+1}-v^*_{j+1}) \sum\limits_{i=1}^j (p_i-p^*_i)  + (v_{j+1} -
    %     v^*_{j+1})(p_{j+1}-p^*_{j+1})\\
    %     = & (v_{j+1}-v^*_{j+1})\sum\limits_{i=1}^{j+1} (p_i-p^*_i)  
    % \end{align*}
\end{proof}
Lemma~\ref{lem: descent direction} shows that given $v$, $-(\oraclep(v) - \optp)$ is always
a descent direction, even though the gradient $\nabla L(v)$
is not necessarily in the same direction as $\oraclep(v)-\optp$. 
% This observation might be of independent interest in other optimization problems
% where this kind of property holds.
Armed with Lemma~\ref{lem: descent direction}, we design a new algorithm for
finding the optimal shift vector by moving in the direction of
$-\oraclep(v)+\optp$ in each step. 
The new algorithm is presented in
Algorithm~\ref{algo: Constant Stepsize Normal Partition Matching}.

% Then we can try to mimic the analysis in \cite{hazan2015beyond}.
\begin{algorithm}
    \DontPrintSemicolon % Some LaTeX compilers require you to use \dontprintsemicolon instead
    \KwIn{Distribution $\cD$, and target matching distribution $p$. Initial
    shift vector $v=[0,\ldots,0]$. Learning rate $\eta$.}
    \For{$t \gets 0, 1, 2, \ldots, T$} {
      $v_{t+1} = v_t - \eta (\oraclep(v_t) - \optp)$\;
    }
    \KwRet{$\bar v_T = \argmin_{\{v_1,\ldots, v_T\}} L(v_t)$}\label{step: argmin in constant step algo}
    \caption{Constant Step Size Normal Partition Matching}
    \label{algo: Constant Stepsize Normal Partition Matching}
\end{algorithm}

In typical optimization literature, a zeroth-order optimization method would
only have access to a function evaluation oracle, which is
$L(v) = ||\oraclep(v)-\optp||_1$ in our case. A first-order optimization method would
have access to the gradient oracle, which is $\nabla L(v)$. 
In contrast, we only require oracle access to $\oraclep(v)$, which is in between
a zeroth-order and first-order oracle. This insight might be of independent
interest in other optimization problems. Our main result for this section is the
following bound on the number of iterations it takes for Algorithm~\ref{algo: Constant Stepsize Normal Partition Matching} to find an approximate solution.

\begin{theorem}
    Algorithm~\ref{algo: Constant Stepsize Normal Partition Matching} with step
    size $\eta = \frac{1}{2n\bar\mu}$ finds an
    $\epsilon$ optimal point (i.e., $L(v) \leq \epsilon)$ within $T =
    \frac{4n^3\bar\mu^2||v_0-v^*||^2_2}{\epsilon^2}$ iterations.
    \label{thm: constant step size convergence result}
\end{theorem}
\begin{proof}
    % Assuming that the shift vector $v_t$ is such that $||\tilde p(v_t) -
    % p||_1 \geq \epsilon$ for $t=1,\ldots, T$, then
    We use $\oraclep_t$ to denote $\oraclep(v_t)$.
    \begin{align*}
    &||v_{t+1} - v^*||^2 \\
    (\text{Algebra})=& ||v_t - v^*||^2 - 2\eta \langle v_t-v^*, \oraclep_t - \optp \rangle + \eta^2 ||\oraclep_t - \optp||_2^2\\ 
    (\text{Lemma~\ref{lem: descent direction}})\leq& ||v_t - v^*||^2 - \eta \frac{||\oraclep_t - \optp||_1^2}{n\bar \mu} + \eta^2 ||\oraclep_t - \optp||_2^2\\ 
    (||\cdot||_2 \leq ||\cdot||_1)\leq& ||v_t - v^*||^2 + ||\oraclep_t - \optp||^2_2 \left(- \frac{\eta}{n\bar \mu} + \eta^2\right)\\ 
    (\text{Set $\eta = \frac{1}{2n\bar\mu}$})=& ||v_t - v^*||^2 - \frac{||\oraclep_t - \optp||^2_2}{4n^2\bar\mu^2}
    \end{align*}
    After rearranging and summing over $t=1, \dots, T-1$, we have
    \begin{align*}
        ||v_0 - v^*||^2 - ||v_T-v^*||^2 \geq \sum_{t=1}^{T-1} \frac{||\oraclep_t
        - \optp||_2^2}{4n^2\bar\mu^2}
    \end{align*}
    Suppose $||\oraclep_t - \optp||_1\geq \epsilon$ for $t=1,\ldots, T$, then
    $||\oraclep_t - \optp||_2^2 \geq\frac{\epsilon^2}{n}$ for $t=1,\ldots, T$.
    This means that
    $T \leq \frac{4n^3\bar\mu^2||v_0-v^*||^2_2}{\epsilon^2}$. 

    % \mycomment{
    % If we can further bound $||v_t-v^*|| \leq C ||\tilde p-p||$, then The
    % convergence is $O(n^2\log(\frac{1}{\epsilon}))$}

\end{proof}

Note that Algorithm~\ref{algo: Constant Stepsize Normal Partition Matching} also
gives rise to a natural \emph{stochastic} optimization algorithm, where in each iteration $t$, instead
of using the exact matching distribution $\oraclep(v_t)$ to find the update
direction, we can use a noisy version $\hat p(v_t)$ to perform the updates.
One natural choice for $\hat p_t$ would be $\hat p(v_t) = [\1(i \text{ is matched
under } v_t)]$ for a randomly drawn item $X\sim\cD$.  It is easy to see that
$\bbE[\hat p(v_t)] = \oraclep(v_t)$. 
In convex optimization, first order methods are known to be very robust and
stochastic variations of the same optimization method usually achieve good
guarantees (e.g., stochastic gradient descent vs gradient descent).
However, since the loss function $L(v)$ in our case is not convex with respect
to $v$, it is difficult to get performance guarantee on the average iterate 
$\frac{1}{T}\sum_{t=1}^T v_t$ or the last iterate $v_T$, as typically seen in
convex optimization literature.


==> NeurIPS 22/Experiments.tex <==
\begin{figure*}[]
	\begin{minipage}{0.33\textwidth}
	    \centering
	    \includegraphics[width=1\textwidth]{artificial_allocation_epsilon0.2.png}
	    % \label{fig: 2D partition}
	\end{minipage}%
	\begin{minipage}{0.33\textwidth}
	    \centering
	    \includegraphics[width=1\textwidth]{artificial_allocation_epsilon0.1.png}
	    % \label{fig: 2D augmenting flow}
	\end{minipage}%
	\begin{minipage}{0.33\textwidth}
	    \centering
	    \includegraphics[width=1\textwidth]{artificial_allocation_epsilon0.0.png}
	    % \label{fig: 2D augmenting flow}
	\end{minipage}
	\caption{Allocation policy for artificial data under different envy
	constraints. From left to right: $\epsilon=0.2, 0.1, 0.0$. When the envy
	constraint is loose (large $\epsilon$), $B$ envies $A$, since both agents
	prefer the items on the top right, but most of them are allocated to $A$. 
	As the envy constraint tightens, the allocation boundary tilts in the
	direction that makes the allocations more even between the two agents.
	}
	\label{fig: slanted dist allocation plot}
\end{figure*}
\begin{figure*}
	\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=0.8\columnwidth]{twodists_tradeoffcurve.png}
    \caption{The trade-off curve between envy and welfare for both data-sets.
    The shaded region is between 25th and 75th percentile of the trials.  The
    non-monotonicity in the plot for the simulator data is due to the
    stochasticity in the SGD algorithm. } 
    \label{fig: slanted dist trade off curve}
	\end{minipage}%
	\hfill
	\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=0.8\columnwidth]{samplecomplexityplot.png}
    \caption{Approximation gap with respect to sample size. Both $x$ and $y$ axis are in log scale. The solid line is the median and the shaded region is between the $25$th and $75$th percentile.  The dashed lines show what the theoretical $1/\sqrt{m}$ rate would look like.}
    \label{fig: sample complexity plot}
	\end{minipage}
\end{figure*}
We test our solution with both artificial data, and simulated data from a realistic
simulator for blood donor matching developed by \cite{mcelfresh2020matching}. The artificial data contains two recipients, and their valuation distribution is a linearly transformed uniform distribution. This is to make visualization of the resulting allocation policy easier. The simulator data is based on geographical and population information from San Francisco, and contains $5$ recipients.
To set the envy budgets $\lambda\in\bbR^n$, we first decide on a constant
$\epsilon \in \bbR_+$, and then multiply this by the target matching
distribution $\optp \in \bbR^n$: $\lambda_{ij} = \epsilon \optp_i\,\forall
i,j$. 
With this setup $\epsilon$ is a bound on the 
normalized envy for each recipient: $\frac{1}{\optp_i}Envy(i)\leq \epsilon \,\forall i.$
Figure~\ref{fig: slanted dist allocation plot} illustrates how the allocation policy changes as we change $\epsilon$. As the envy constraint tightens, the decision boundary tilts in the direction that split the ``good'' (items which both agents prefer) and ``bad'' (items which both agents dislike) items more evenly between the recipients.


Next we investigate the trade-off between envy and social welfare by using SGD to
compute approximately optimal allocations for varying $\epsilon$.  We plot the
percent welfare gap (difference between the maximum welfare without envy
constraints, and the welfare with envy constraints, divided by the former) with
respect to realized, max normalized envy.  Figure~\ref{fig: slanted dist trade
off curve} shows the result.  For the simulator data, the welfare gap is small
even with a no-envy constraint, which means that aiming for envy free
allocations might make sense. In the case of the artificial data however, paying
$~50\%$ of the full price of fairness reduces $~65\%$ of the envy. In such
settings, one might want to sacrifice some envy for better welfare.

These experiments also highlight when envy arises. When recipients' utilities are
highly correlated, but one recipient has larger variance than others, that
recipient receives almost all the good items (which results in large envy for
other recipients), even though others value the items almost as much. In such
cases, a small reduction in welfare can reduce a large amount of envy. This
seems to be the case for the simulator data. On the other hand, if utilities are
correlated, but only one recipient has very strong preferences, then allowing a
small amount of envy can improve the welfare significantly.



Finally, in Figure~\ref{fig: sample complexity plot} we investigate the quality
of the empirical solutions as the sample size increases. It can been seen that
the approximation gap decreases faster than the theoretical rate, confirming our
sample complexity bound in Theorem~\ref{thm: sample complexity bound}. 

\section{Limitations and Future Directions}
\label{sec: future directions}
Although we believe that the model proposed here is natural, and captures the
most salient aspects of some of the resource allocation problems in real life, 
any implementation of our proposed strategy in critical applications such as 
blood donation should be prefaced with more rigorous backtesting in order to
minimize the risk of unintended consequences in application specific metrics not
studied in this paper.

For future directions, one key property that we did not study in this paper is
the problem of incentive compatibility. For our motivating application of blood
donation, this is not an issue because online platforms such as Meta has
proprietary models that can predict the matching quality between donor and
recipient. This means that the platform observes the value of matchings without
having to rely on the recipients to self-report. This is also true in many other
online matching problems such as sponsored ads. However, in settings where the
central planner relies on the recipients to self-report their valuations for each
of the items, incentive compatibility becomes a crucial issue. We are excited
about the potential of using Optimal Transport in fair-division, and plan on
exploring the incentive issues in future work.


% \begin{figure*}[]
% 	\begin{minipage}{0.33\textwidth}
% 	    \centering
% 	    \includegraphics[width=0.9\textwidth]{simulator_dist_epsilon0.1.png}
% 	    % \label{fig: 2D partition}
% 	\end{minipage}%
% 	\begin{minipage}{0.33\textwidth}
% 	    \centering
% 	    \includegraphics[width=0.9\textwidth]{simulator_dist_epsilon0.05.png}
% 	    % \label{fig: 2D augmenting flow}
% 	\end{minipage}%
% 	\begin{minipage}{0.33\textwidth}
% 	    \centering
% 	    \includegraphics[width=0.9\textwidth]{simulator_dist_epsilon0.0.png}
% 	    % \label{fig: 2D augmenting flow}
% 	\end{minipage}
% 	\caption{For the simulated blood donation data it is more difficult to
% 	see visually the difference between different envy constraints. However
% 	we can see that as the envy constraint gets tighter, welfare drops.}
% 	\label{fig: simulator dist allocation plot}
% \end{figure*}





==> NeurIPS 22/Introduction.tex <==
% There has been growing interest in resource allocation algorithms for online
% problems, driven by a variety of applications in e-commerce, advertising, and
% more.  Many works have focused on the ``online performance'' of the algorithms
% as measured by the difference between what the best value (e.g., revenue,
% utility, welfare) one can achieve knowing the sequence/distribution of
% items/requests ahead of time, often referred to as the offline solution, and the
% value that the algorithm is able to achieve without this clairvoyant knowledge.
% Surprisingly, few have tried to understand the structure of the offline optimal
% solution.  This is partially due to the fact that many of the analysis done in
% these prior works need not consider the optimal offline solution explicitly.
% However, modeling resource allocation problems as an online problem does not
% always make the most sense.  For example, when there is historical data
% available, and the problem is relatively stationary (i.e. the past is predictive
% of the future), it would be wasteful to not utilize the data available and
% instead ask an algorithm to start from scratch and learn everything in an online
% fashion.  Additionally, online algorithms require dynamically updating
% parameters, which requires significantly more advanced engineering
% infrastructure that only established companies with the engineering resources
% can afford to implement in practice.

In this work, we focus on the problem of finding an allocation policy that
divides a pool of items, represented by a distribution $\cD$, to $n$ recipients,
under the constraint that each recipient $i$ must be allocated a pre-specified
fraction $\optp_i$ of the items, where $\optp_i\in(0,1), 1^\top \optp = 1$ is an
input to the problem that characterizes the priority of each recipient. We refer
to $\{\optp_i\}_{i=1}^n$ as the target matching distribution. In addition to
this matching distribution constraint, we also require that the recipient's envy,
which we will define formally later, be bounded. Unlike the existing resource
allocation literature, where envy-free is either treated as a hard constraint or
not considered at all (in divisible settings), we allow the central planner to specify the level of envy
that is tolerated, and find the most efficient allocation given the amount of
envy budget. This allows us to reduce the envy significantly without paying the
full price of fairness with respect to efficiency.

To concretely motivate our model, let us consider the blood donor matching
problem that was first studied in \cite{mcelfresh2020matching}.  The Meta
platform has a tool called \emph{Facebook Blood Donations}, where users who opt
in to receive notifications are notified about blood donation opportunities near
them.  Depending on the user's and the blood bank's specific characteristics
(e.g., age, occupation for the user, and locations, hours for the blood bank),
notifications about different donation opportunities have different
probabilities of resulting in an actual blood donation. The platform would like
to send each user the most relevant notifications (to maximize the total number
of potential blood donations), while maintaining certain fairness criteria for
all the blood banks that participate in this program. Although the platform can
theoretically send each user multiple notifications about multiple blood banks,
for user experience and other practical reasons, this is not done, at least in
the model introduced in \cite{mcelfresh2020matching}.  Therefore in this
problem, users' attention is the scarce resource that the platforms needs to
allocate to different blood banks. The most natural type of fairness criteria in
this setting is perhaps the number of users that received notifications about
each of the blood banks.  For example, it is not desirable to match zero users
to a particular, potentially inconveniently-located, blood bank, even if
matching zero users to this blood bank results in more blood donations in
expectation.  

Another fairness desideratum commonly studied in the
literature is called \emph{envy-freeness}. We say that recipient $A$ envies recipient $B$
if $A$ values $B$'s allocation more than her own. Intuitively, an allocation
that is envy-free--where no agent envies another agent--is perceived to be fair.

This paper considers both of the two fairness criteria mentioned above:
we study a setting where the goal is to maximize social welfare under a matching distribution constraint, while ensuring that each recipient has bounded envy.
We make the following contributions in regards to this problem:
\begin{enumerate}
    \item We formulate it as a constrained version of a semi-discrete optimal
    transport problem and show that the optimal allocation policy has a concise
    representation and a simple geometric structure. 
    This is particularly
    attractive for large-scale allocation problems, due to the fast computation
    of a match given an item. This insight also shines new light on the question of when envy arises, and when the welfare price on envy-freeness is large. 
    \item We propose an efficient stochastic optimization algorithm for this
    problem and show that it has a provable convergence rate of $O(1/\sqrt{T})$.
    \item We investigate the statistical properties of the space of our
    optimal transport based allocation policies by showing a Probably Approximately Correct (PAC)-like sample
    complexity bound for approximating the optimal solution given finite
    samples. 
\end{enumerate}

In Section~\ref{sec: problem formulation} we formally define the problem we are interested in. In Section~\ref{sec: solution structure}, we show that this problem can be
formulated as a semi-discrete optimal transport problem, whose solution has a
simple structure with a nice geometric interpretation. 
Section~\ref{sec: stochastic optimization} develops a practical stochastic optimization algorithm.
In
Section~\ref{sec: learning from samples}, we show that an $\epsilon$-approximate
solution can be found with high probability given $\tilde
O(\frac{n}{\epsilon^2})$ samples, where $n$ is the number of
recipients. Finally, in Section~\ref{sec: experiments} we demonstrate the effectiveness of our approach using both artificial and a semi-real data.


\section{Literature Review}
\paragraph{Blood donation matching.}
\textcite{mcelfresh2020matching} introduced this problem and modeled it as  an
online matching problem, where the matching quality between an user and a blood
bank is assumed to be known to the platform. The model formulation there is complex and their matching policy is rather
cumbersome, requiring a separate parameter for each (donor, recipient) pair.
Compared to their paper, we are able to provide better
structural insights to the problem by utilizing a simpler model that still
captures the most salient part of the problem.


% , and our matching policy can be
% represented by just $n$ parameters, where $n$ is the number of recipients.
\paragraph{Online Resource Allocation.}
%% Short version of the Online resource allocation lit review
\iffalse
Another strand of work that our paper is closely related to is that of online
resource allocation, especially those with i.i.d. or random permutation input
models~\cite{goel2008online,devanur2009adwords,devanur2019near,agrawal2014dynamic,agrawal2014fast,balseiro2020best}. 
However, none of theses papers study the concept of envy.
Recently, \textcite{balseiro2021regularized} studied an online resource allocation
problem with fairness regularization. Although envy regularization can be formulated in their framework, they did not provide an explicit solution to the offline problem. Our analysis focuses
on the offline problem, and draws an explicit connection to optimal transport,
which allowed us to provide a novel PAC-like analysis on the sample complexity
of the problem. 
\fi

Another strand of work that our paper is closely related to is that of online
resource allocation, especially those with i.i.d. or random permutation input
models. \textcite{agrawal2014dynamic} studied the setting with linear objective and gave
competitive ratio bounds. Then, \textcite{agrawal2014fast} generalized the results to
concave objectives and convex constraints. Later, \textcite{devanur2019near}
improved the approximation ratio bounds and relaxed the input assumptions on the
budgets. \textcite{balseiro2020best} show that online mirror descent on the dual
multipliers does well under both i.i.d. adversarial, and certain non-stationary
input settings.
However, none of theses papers study the envy-free criterion.
Recently, \textcite{balseiro2021regularized} studied an online resource allocation
problem with fairness regularization. Although the authors did not explicitly
study envy regularization, their regularization framework can be modified to
accommodate envy regularization. However, like all the other papers mentioned in
this paragraph, the offline solution is used as the benchmark to measure regret,
but no explicit solution is given to the offline problem. Our analysis focuses
on the offline problem, and draws an explicit connection to optimal transport,
which allowed us to provide a novel PAC-like analysis on the sample complexity
of the problem. In another recent paper, \textcite{sinclair2021sequential} studied
the trade-off between minimizing envy and minimizing waste, which refers to un-allocated resources. Despite close similarity between our titles, their offline benchmark
is the standard Eisenberg-Gale program, which is envy-free, but does not address
the welfare cost of achieving envy-freeness. 
\paragraph{Fair Division.}
Envy is a popular concept studied in the fair division literature. A large body of these papers are formulated as a
cake-cutting problem (\cite{robertson1998cake,chen2013truth,mossel2010truthful})
where the resources are modeled as an interval and the agents' valuations are
represented as functions on this interval. 
\textcite{caragiannis2009efficiency} provide a analysis on the worst case efficiency loss due to the envy-freeness constraint. Later \textcite{cohler2011optimal} design algorithms for computing optimal envy-free cake cutting allocations under different relatively simple classes of valuation functions. 
Unlike these papers that focus on the hard constraint of zero envy, we treat the allowable envy as a parameter, and find the most
efficient solutions subject to the desired amount of envy.
In indivisible settings, there are some related concepts of envy that does not require a strict zero envy. For instance, \textcite{budish2011combinatorial} proposes an approximate competitive equilibrium from equal incomes approach that  achieves envy free up to 1 item (EF1). \textcite{caragiannis2019unreasonable} introduce the concept of envy free up to the Least Valued Good, which is a stronger version of EF1. Although these papers do allow a small amount of envy, these concepts are introduced mainly to circumvent the impossibilities introduced by the indivisible settings, not to allow central planners to control the level of envy tolerance. Finally, \textcite{donahue2020fairness} also studies a setting where the central planner can set his own tolerance of (un)fairness. However their setting is quite different from ours, as they consider the allocation of fixed amount of identical resource, where as we assume that recipients have different valuations for the different items.

\paragraph{Optimal Transport.} OT has been applied before in resource allocation settings in the economics literature (see \cite{galichon2018optimal} for a survey). 
For example, the Hotelling location model with a continuous mass of consumers can be solved with the same assignment procedure as the one we consider for our allocation problem \emph{without} envy constraints. The more general method of assigning points in space to a finite set of sites via this procedure was developed by \textcite{aurenhammer1998minkowski}.
\textcite{scetbon2021equitable} consider an OT setting with equitability (every agent's final utility is the same), which is a different fairness criteria from envy, and also not adjustable like in our setting. To the best of our knowledge, no existing application of OT models the envy constraints that we consider here.

% their model is completely different, as they consider a classical OT problem with an \emph{auxiliary} set of agents that have preferences over the specific transportation map being chosen.

%  These papers often focus on properties such as
% proportionality (i.e., whether each recipients gets $1/n$ fraction of the
% value according to their own utility functions), envy-freeness (i.e., whether
% some recipient wish that they received the allocation of someone else's), or
% strategy-proofness (i.e., whether a recipient can get more allocation by
% misreporting their utility function). 


% For example, \cite{cohler2011optimal} proposes an
% algorithm for finding the most efficient allocation subject to the envy-free
% constraint in the cake cutting setting. 

% The first difference between these papers
% and ours is that they do not study the budget constraint we consider here (i.e.,
% the constraint that each recipient receives $\optp_i$ fraction of the ``cake''). 
% Additionally, 
% In other words, our formulation can be more accurately described as
% the offline version of the recent strand of online resource allocation papers
% mentioned above, rather than an extension of the much older research on 
% cake-cutting.

% \paragraph{Optimal Transport}
% Our problem can also be viewed as an optimal transport problem
% \cite{santambrogio2015optimal}, where the we try to transport the initial
% distribution of items, to a discrete distribution of $n$ point masses, each with
% a pre-specified amount. However, most results in this area deal with cost 
% functions with simple structures, and cannot be directly utilized in our
% problem. Lastly, as we will describe later, our problem can be thought of as a
% non-convex optimization problem.  To that end, some of our analysis resembles
% that seen in \cite{hazan2015beyond}, which studies a gradient based, stochastic quasi-convex optimization algorithm. However, the underlying structures that
% made the analysis possible are fundamentally different, since we do not even require
% access to a gradient oracle.
% The update direction that we use in Algorithm~\ref{algo:
% Constant Stepsize Normal Partition Matching} has an intuitive interpretation in
% our setting. 




\subsection{Background on Optimal Transport}
Since our work draws an explicit connection to optimal transport (OT), we provide a
summary of key OT results here.  Let $\alpha, \beta$ be two probability measures on
the metric spaces $\cX, \cY$ respectively. We define $\Pi(\alpha, \beta)$ as the
set of joint probability measures on $\cX\times \cY$ with marginals $\alpha$ and
$\beta$. The \emph{Kantorovich formulation} of the optimal transport problem
\cite{kantorovich1942on} can be written as
\begin{align}
     L(\alpha, \beta)\coloneqq \min_{\pi \in \Pi(\alpha, \beta)}\int_{\cX \times \cY} c(x, y) d\pi(x, y)
    \label{eq: optimal tranport primal}
\end{align}
where $c(x, y)$ is the cost associated with ``moving'' $x$ to $y$.  This is
called a transportation problem because the conditional probability $\pi(y|x)$
specifies a transportation plan for moving probability mass from $\cX$ to $\cY$. Note that $\pi(x, y) = \pi(y|x)d\alpha(x)$.
If $\beta$ is a discrete measure, i.e. $\cY$ is finite, then it is known
\cite{aude2016stochastic} that the dual to \eqref{eq: optimal tranport primal}
can be written as (here we abuse the notation $\beta$ to also represent the
vector of probability masses, where $\beta_i$ is the probability mass on point
$y_i$):
\begin{equation}
    \max_{g\in\bbR^n} \cE(g) \coloneqq \sum_{i\in[n]}\left[\int_{\bbL_{y_i}(g)} c(x, y_i)-g_i\,d\alpha(x)\right] + g^\top \beta
    \label{eq: optimal transport dual}
\end{equation}
where $n=|\cY|$, and $\bbL_{y_i}$ is what is sometimes referred to as the \emph{Laguerre
cell}: 
\begin{equation}
\bbL_{y_i}(g) = \left\{x\in\cX: \forall i\neq j, c(x, y_i) - g_i\leq c(x, y_j)-g_{j} \right\}
\label{eq: laguerre cell}
\end{equation}
\begin{proposition}[Proposition~2.1 \cite{aude2016stochastic}]
    If $\alpha$ is a continuous measure, and $\beta$ a discrete measure, then
    $L(\alpha, \beta) = \max\limits_{g}\cE(g)$, and
    the optimal solution $\pi$ of \eqref{eq: optimal tranport primal} is given by the partition $\left\{\bbL_{y_i}(g^*), i\in
    [n]\right\}$, i.e. $d\pi(x, y_i)=d\alpha(x)$ if $x\in \bbL_{y_i}(g^*)$, $0$ otherwise.
    \label{thm: duality of semi-discrete OT}
\end{proposition}




==> NeurIPS 22/LearningFromSamples.tex <==
So far we have assumed that the true underlying distribution is
known, and that we can freely draw independent samples it.
In many settings, we only have access to $\alpha$
in the form of finite number of i.i.d. samples. The goal of this section is to establish a sample complexity bound for solving the dual problem
$\eqref{eq: individual envy constraint dual laguerre}$. 


% This complements the result in the previous section by providing an algorithm agnostic bound on the sample complexity.
% To build some intuitions for how we are able to derive the result in this section, readers familiar with traditional PAC learning results might recall that hyperplanes have a low VC-dimension. 
% Similar to how low VC-dimension leads to low sample complexity in classification tasks, the fact the boundaries of our Laguerre cells are consisted of hyperplanes also lead to low sample complexity in our setting.

In this section, we focus only on the assignment cost function $c(x, y_i) =
-x_i$, which models our original resource allocation problem proposed in Section~\ref{sec: problem formulation}.
Let $S = \{X^1, X^2, \ldots, X^m\}$ be $m$ independent samples from
$\alpha$. The empirical version of the dual objective \eqref{eq: dual objective
integration version} is:
\begin{equation}
    \label{eq: dual objective empirical}
    \cE_S(g, \gamma) = \frac{1}{m} \sum\limits_{t=1}^m\min_{i\in [n]} \dualg(X^t, y_i) + g^\top \beta - \sum_{j,k, j\neq k}\gamma_{jk}\lambda_j
\end{equation}
Let $\hat g_S, \hat \gamma_S$ be the empirical maximizer given the set of
samples $S$: $(\hat g_S, \hat\gamma_S) \coloneqq \argmax \cE_S(g, \gamma)$, and
$g^*, \gamma^*$ be the population maximizer $(g^*, \gamma^*)=\argmax \cE(g,
\gamma)$.
% Let $\hat p_S(g)$ be the empirical matching distribution given the
% dual variables $g, \gamma$
% : $$\hat p_S(v)_i = \frac{1}{m}\sum_{k=1}^m \1\left[ i = \bbL_{y_i}(g, \gamma) \min
% \left(\argmax_j X^{k}_j+v_j\right)\right]$$ We take the standard approach in
% learning theory, and let our estimator given set $S$ be the one that minimizes
% the loss on the empirical distribution:
% $$v(S) = \argmin_v ||\hat p_S(v) - p||_1$$
% We switch to the $L1$ norm for ease of analysis. Since $||\cdot||_1\geq
% ||\cdot||_2$, the bound can be easily converted to one for the original loss
% function \eqref{eq: minimizing square loss} as well.
% Note that the setting is different from the standard learning theory setting, as
% the true loss function cannot be written as the expectation of the empirical loss function:
% $$||p(v) - p^*||_1 \neq \bbE_{S\sim \alpha}\left[||\hat p_S(v) - \optp||_1\right]$$
% We are interested in the number of samples needed so that $\oraclep(v(S))$ is close to
% $\optp$. Let us state our main result first.
We want to bound the number of samples needed so that $\cE(g^*,
\gamma^*) - \cE(\hat g_S, \hat \gamma_S)$ is small with high probability.  Let's
introduce some notations to facilitate our later discussions.  Define the
following hypothesis class for each $i$:
\begin{align}    
    F_i = \left\{x\mapsto \dualg(x, y_i) + g^\top \beta - \sum_{j,k, j\neq k}\gamma_{jk}\lambda_j: g \in \bbR^n, \gamma \in \bbR_+^{n(n-1)}\right\}.
    \label{eq: separate hypothesis class definition}
\end{align} 
as well as the overall hypothesis class:
\begin{align}    
    F = \left\{x\mapsto \min_{i\in[n]}\dualg(x, y_i) + g^\top \beta - \sum_{j,k,
    j\neq k}\gamma_{jk}\lambda_j : g \in \bbR^n, \gamma \in
    \bbR_+^{n(n-1)}\right\}.
    \label{eq: hypothesis class definition}
\end{align} 
Plugging $c(x, y_i) = -x_i$ into the definition of $\dualg$, we see that for a given $g, $ and $\gamma$, the corresponding
hypothesis $f_i\in F_i$ can be written as $f_i(x) = w^\top x + b$, where 
\begin{equation}
    \label{eq: w definition}
w_j = 
  \begin{cases}
    -(1+\sum\limits_{k\neq i}\gamma_{ik}), &\text{if $j=i$}\\
    \gamma_{ji}\frac{\beta_j}{\beta_i}, &\text{if $j\neq i$}
  \end{cases}, \text{ and} 
\end{equation}
\begin{equation}
    \label{eq: b definition}
b = -g_i + g^\top \beta -  \sum_{j,k,
j\neq k}\gamma_{jk}\lambda_j.
\end{equation} 
It also follows that 
\begin{equation}
    \label{eq: hypothesis class contained in the min over halfspaces}
    F \subseteq F_{min} \coloneqq \{x\mapsto \min_i f_i(x): f_i\in F_i\}.
\end{equation}
Note that $F$ defined in \eqref{eq: hypothesis class definition} is the main object of interest, as it contains all the possible Laguerre cell parameters.  We showed in \eqref{eq: hypothesis class contained in the min over halfspaces} that $F$ is at most as complex as $F_{min}$, a hypothsis class constructed from $n$ affine hypothesis classes. This interpretation of the original hypothesis class as the minimum over $n$
affine hypothesis classes is the key observation to prove the sample complexity
bound.  We prove our main result under the following boundedness assumption:
\begin{assumption}
    The hypothesis $f(x) = \min_i f_i(x) = \min\limits_i {w^i}^\top x +b^i$ corresponding to the optimal dual solution $g^*,
    \gamma^*$ satisfies $\|w^i\|_1\vee |b^i| \leq R$ for some $R>0$. In particular,
    these assumptions imply that $F_i$ and $F$ are uniformly bounded by $R\bar x + R$.
    \label{assum: boundedness assumptions}
\end{assumption}
From \eqref{eq: w definition} and \eqref{eq: b definition} we can see that this
is essentially a bound on the optimal dual variables $g^*, \gamma^*$, and a
bound on the ratio $\beta_j/\beta_i$, both of which are determined by the input
distributions $\alpha, \beta$, and do not depend on the number of samples. In
other words, $R$ is a problem dependent constant.

\begin{theorem}
Under Assumption~\ref{assum: boundedness assumptions}, for a given sample size $m$, 
with probability $1-\delta$,  $\cE(g^*, \gamma^*)
- \cE(\hat g_S, \hat \gamma_S) < O\left(\sqrt{\frac{(\log m)^3 + \log(1/\delta)}{m}}\right)$. 
\label{thm: sample complexity bound}
\end{theorem}
The proof of this theorem can be found in the appendix. We will provide some high level intuition here. The proof uses the fat-shattering dimension, which is a concept that generalizes the Vapnik–Chervonenkis (VC) dimension to functions of real values. Like the VC dimension, the fat-shattering dimension is a measure of capacity for a class of functions. The larger the fat-shattering dimension, the more ``complex'' the function class is. Intuitively, the more complex the function class is, the more samples one needs to accurately identify the optimal function within that class. Recall that the object of interest in our paper is the Laguerre cell, whose boundaries are defined by a set of hyperplanes. Readers readers familiar with traditional PAC learning results might recall that hyperplanes have a low VC dimension. It turns out that the hypothesis class associated with Laguerre cells defined above in \eqref{eq: hypothesis class definition} has a low complexity as well. 
Similar to how low VC dimension leads to low sample complexity in classification tasks, the fact the boundaries of our Laguerre cells are consisted of hyperplanes also lead to low sample complexity in our setting.

\paragraph{Relation to Section~\ref{sec: stochastic optimization}} Note that there is some connection between the convergence of a stochastic optimization method (computational complexity), and the sample complexity bound of the same problem (learning complexity). Both say something about the number of steps/samples one needs to arrive at a good solution. However, in general, these two things are not the same. In particular, the learning complexity result from this section is algorithm agnostic. The proof of Theorem~\ref{thm: sample complexity bound} actually implies uniform convergence: that no matter which hypothesis one considers, its' empirical objective will be close to the expected objective. However, Theorem~\ref{thm: sample complexity bound} does not provide a way for practitioners to actually compute the solution. The result from Section~\ref{sec: stochastic optimization} on the other hand does provide an algorithm for practitioners to use, and shows that the algorithm is computationally efficient. However, the convergence result  in Section~\ref{sec: stochastic optimization} only works for the specific optimization method that we proposed. Therefore these two results are complements of each other, and together paint a relatively complete picture on how difficult the task it.
% Note that Assumption~\ref{assumption: regularity of the distribution} is a
% sufficient condition for an optimal normal partition to exist (by
% Lemma~\ref{lem:unique normal partition}), but may not be necessary. The
% following proof does not need the regularity conditions in
% Assumption~\ref{assumption: regularity of the distribution} other than the
% existence of a normal partition $v^*$ such that $p(v^*) = \optp$.



==> NeurIPS 22/ProblemFormulation.tex <==
There is a set of $n$ recipients $\cY$. There is a ``pool'' of items,
represented by a distribution $\alpha$ over $\cX\subseteq [0, \bar x]^n$. Each
random draw from this distribution $X\sim \alpha$ is a vector representing the
$n$ recipients' valuations of this item. The goal is to maximize the expected
matched utilities of the recipients, while maintaining the constraint that the
recipient $y_i$ is matched $\optp_i$ fraction of the times in expectation.  Here
$\{\optp_i\}_{i=1}^n$ is called the target matching distribution, which
intuitively represents recipients' importance. Note that the constrains here are satisfied \emph{in expectation}, which are sometimes referred to as ``ex-ante'' guarantees.  The reason why we consider ex-ante guarantees has to do with the type of application we're interested in. Our motivating example is concerned with recommending hundreds of millions of users to different blood banks. In such settings, even if we want the constraints to hold ex-post, the large-scale nature of the problem and the law of large numbers means that in-expectation guarantees translate into something that is very close to holding ex-post. That is why for internet platform problems, requiring constraints to hold in expectation is a  standard setup (see for example the literature on budget constraints in ad auctions, where this is the case \cite{balseiro2015repeated}). A matching policy $\pi$ takes a
valuation vector and maps it (potentially with randomness) to one of the $n$
recipients. Let $\pi(y|x)$ denote the probability of matching the item to $y$
given valuation vector $x$. The basic problem formulation is to solve the
following optimization problem:
\begin{align}
    \max\limits_{\pi}\,&\bbE_{X\sim\alpha}\left[ \sum_{i=1}^n X_i\pi(y_i|X)]\right]\label{prob: basic optimal matching policy problem}\\ 
    s.t.\quad & \bbP\left[\pi(y_i|X)\right] = \optp_{i}\quad \forall i\in[n]\nonumber
\end{align}
WLOG, we assume that $\optp_i>0$ for all $i$. An example of such problem can be see in Figure~\ref*{fig: 2D
example}, where $\alpha$ is a distribution over the unit square, and the goal is
to partition the square into blue and orange regions (given to $A$ and $B$
respectively) such that each region covers the desired $p^*_A$, $p^*_B$
probability mass. Note that the orange and blue regions are allowed to over lap
(probabilistic partition), and that the boundary does not have to be linear as
illustrated in the figure. As we will show later in Section~\ref{sec: solution
structure}, despite the large design space permitted by the formulation in
\eqref{prob: basic optimal matching policy problem}, we can in fact focus on a
much smaller design space. 

In resource allocation problems, it is often the case that we care not just
about efficiency (the sum of all recipients'
utilities), but also other fairness criteria.  One of the most commonly studied
fairness criteria is envy-freeness. Agent $y_i$ envies another agent $y_j$ if agent
$y_i$ values the allocation given to $y_j$ more (after adjusting for their priority
weights). We can formally define agent $y_i$'s envy as 
\begin{equation}
    \label{eq: envy definition}
    % Envy(i) = \max_k \int_{\cX}c(x, j) d\pi(x, j) - \int_{\cX}c(x, j) d\pi(x, k) \frac{\beta_j}{\beta_k} 
    Envy(y_i) = \max_j \bbE_{\alpha}\left[ X_i\pi(y_j|X) \frac{\optp_i}{\optp_j} - X_i\pi(y_i | X)\right]
\end{equation}
Instead of the vanilla formulation in \eqref{prob: basic optimal matching policy
problem}, we consider the following more general formulation:
\begin{align}
    \max\limits_{\pi}\,&\bbE_{X\sim\alpha}\left[ \sum_{i=1}^n X_i\pi(y_i|X)]\right]\label{prob: optimal matching policy problem}\\ 
    s.t.\quad & \bbP\left[\pi(y_i|X)\right] = \optp_i\quad \forall i\in[n]\nonumber\\
    & Envy(y_i)\leq \lambda_i\quad\forall i\nonumber
\end{align}
Most existing literature focuses on finding
allocations such that $Envy(y_i)$ is at most $0$ for every $y_i$. This can be
a very restrictive constraint, often satisfied at the cost of reducing
efficiency by a significant amount (This reduction is sometimes referred to
as the Cost-of-Fairness). We take a different approach, and allow the central
planner to set non-negative constraints on envy. Note that since we are motivated by internet-scale problems such as allocating hundreds of millions of users to donation centers, we focus on the ex-ante guarantees on the constraints. 









==> NeurIPS 22/SolutionStructure.tex <==
The space of feasible solutions for \eqref{prob: optimal matching policy problem} is
large, which makes the problem difficult to optimize directly. However we can
use the tools from OT to reduce the search space to something
with much more structure.  The key observation is that \eqref{prob: optimal
matching policy problem} can be formulated as variation of the semi-discrete
optimal transport problem given in Equation~\eqref{eq: optimal tranport primal}. 

Let's first consider the simpler case in \eqref{prob: basic optimal matching
policy problem} where there are no envy constraints.  In this case, the problem
can be stated in the form of \eqref{eq: optimal tranport primal} as follows: the
cost function is the negative utility of the matched recipient $c(x, y_i) =
-x_i$, the $\beta$ measure is the discrete measure
$\sum_{i=1}^n\optp_i\delta_{y_i}$, and the matching policy $\pi(y|x)$ in
\eqref{prob: optimal matching policy problem} is exactly the conditional
probability of the joint distribution in \eqref{eq: optimal tranport primal}.
From Theorem~\ref{thm: duality of semi-discrete OT} it follows that the optimal
matching policy is represented by Laguerre cells given in \eqref{eq: laguerre
cell}: $x$ is matched to $y_i$ if $i = \argmin_{k} -x_{k} - g_{k}$.
% or equivalently $i = \argmax\limits_{k} x_{k} + g_{k}.$ 
Note that the dual
variables $g\in \bbR^n$ serve as an ``adjustment'' over the agents' reported
utilities, and the resulting matching policy is simply a greedy policy over this
adjusted valuation vector. 
\begin{figure*}[]
\begin{minipage}{0.5\textwidth}
    \centering
    \includegraphics[width=0.65\textwidth]{2d_normal_partition.png}
\end{minipage}%
\begin{minipage}{0.5\textwidth}
    \centering
    \includegraphics[width=0.65\textwidth]{2d_normal_partition_proof.png}
\end{minipage}
\caption{Left: An illustration of what Laguerre cells look like when $n=2$. Consider any distribution on the support $[0,1]^2$.
The optimal division of the space is to move the diagonal line up or down until
the probability mass contained in the orange region is equal to $\optp$. Right:
A pictorial proof of the optimality of such partition.  Suppose one can find an
$\epsilon$ mass above this line that is matched to $A$, and an $\epsilon$ mass
below the line that is matched to $B$, then switching the assignments of these
two regions increases the matched weights because $B_1+A_2 > A_1+B_2$.}
\label{fig: 2D example}
\end{figure*}

Geometrically, each Laguerre cell is simply the intersection of
half-spaces: $\bbL_i(g)=\cap_{k} \{ x: x_i+g_i \geq x_k + g_k\}$. To visualize this
better, consider the simple setting with two recipients $A, B$ where their
valuations for an item is a joint distribution supported on $[0,1]^2$.
Suppose we want to match $\optp$ fraction of the items to recipient $B$.
Figure~\ref{fig: 2D example} gives a proof-by-picture that the optimal strategy
is to divide the space up with a slope-$1$ diagonal line such
that the probability mass lying above the line is equal to $\optp$. This
geometric interpretation of the matching policy plays a crucial role in getting 
us a sample complexity bound later in Section~\ref{sec: learning from samples}.

With this geometric interpretation of the solution space in mind, let us
consider the more general case with envy constraints as formulated in
\eqref{prob: optimal matching policy problem}.  The envy constraints can be
added to the OT problem in \eqref{eq: optimal tranport primal} like so:
\begin{align}
    L(\alpha, \beta, \lambda) =  &\min\limits_{\pi\in \Pi(\alpha,\beta)} \int_{\cX \times \cY} c(x, y) d\pi(x, y)\label{eq: individual envy constraint primal}\\
    s.t. &\int_{\cX}c(x, y_j) d\pi(x, y_j) - \int_{\cX}c(x, y_j) d\pi(x, y_k) \frac{\beta_j}{\beta_k} \leq \lambda_j 
    &\forall (j,k)\in [n]^2, j\neq k\nonumber
\end{align}
Although envy constraints make the solution space more
complicated, we show that it retains the geometric structure of being the
intersection of half-spaces. The dual of \eqref{eq: individual envy constraint
primal} can be derived using Fenchel-Rockafellar's theorem:
% \begin{align}
%     \max_{g\in\bbR^n, \gamma\in\bbR^{n^2-n}_+} \cE(g,\gamma)\coloneqq\int_\cX \dualg(x) d\alpha(x) + g^\top \beta - \sum_{j,k, j\neq k}\gamma_{jk}\lambda_j
%     \label{eq: individual envy constraint dual finite dim}
% \end{align}
% \begin{align}
%     \max_{g\in\bbR^n, \gamma\in\bbR^{n^2-n}_+}\cE(g, \gamma) = \sum_{j\in [n]}\int_{\bbL_{y_j}(g, \gamma)} \left(1+\sum_{k\neq j}
%     \gamma_{jk}\right)c(x, j) - \sum_{k\neq y}\gamma_{kj}c(x,
%     k)\frac{\beta_k}{\beta_j} - g_j d\alpha(x) + g^\top \beta - \sum_{y,k, y\neq k}\gamma_{jk}\lambda_j\label{eq: individual envy constraint dual laguerre}
% \end{align}
\begin{align}
    \max_{g\in\bbR^n, \gamma\in\bbR^{n^2-n}_+}\cE(g, \gamma) \coloneqq &\sum_{j\in [n]}\int_{\bbL_{y_j}(g, \gamma)} \dualg(x, y_j) d\alpha(x)
     + g^\top \beta - \sum_{j,k, j\neq k}\gamma_{jk}\lambda_j\label{eq: individual envy constraint dual laguerre}
\end{align}
where 
% \begin{align}
% \dualg(x, y_j) \coloneqq &\left(1+\sum_{k\neq j}
% \gamma_{jk}\right)c(x, y_j) - \sum_{k\neq j}\gamma_{kj}c(x,
% y_k)\frac{\beta_k}{\beta_j} - g_j,
% \label{eq: dual g with envy}\\
% % and 
% \bbL_y(g, \gamma) \coloneqq &\left\{ x\in\cX: y = \argmin\limits_{y'\in\cY} \dualg(x, y')\right\}.
% \label{eq: generalized laguerre cell}
% \end{align}
\begin{equation}
\label{eq: dual g with envy}
    \dualg(x, y_j) \coloneqq \left(1+\sum_{k\neq j}
\gamma_{jk}\right)c(x, y_j) - \sum_{k\neq j}\gamma_{kj}c(x,
y_k)\frac{\beta_k}{\beta_j} - g_j,
\end{equation}%
\begin{equation}
\label{eq: generalized laguerre cell}
    \bbL_y(g, \gamma) \coloneqq \left\{ x\in\cX: y = \argmin\limits_{y'\in\cY} \dualg(x, y')\right\}.
\end{equation}%


\begin{theorem}
    If $\alpha$ is a continuous measure, and $\beta$ a discrete measure, then
    $L(\alpha, \beta, \lambda) = \max\limits_{g, \gamma}\cE(g, \gamma)$, and
    the optimal solution $\pi$ of \eqref{eq: individual envy constraint
    primal} is given by the partition $\left\{\bbL_{y_i}(g^*, \gamma^*), i\in
    [n]\right\}$: $d\pi(x, y_i) = d\alpha(x)$ if $x\in \bbL_{y_i}(g^*, \gamma^*)$,
    $0$ otherwise.
    \label{thm: duality of envy constrained OT}
\end{theorem}
Note that when $c(x, y_i) = -x_i$, $\dualg(x, y_j)$ is linear in $x$,
which means that the new Laguerre cells $\bbL_y(g, y)$ given in Equation~\eqref{eq: generalized
laguerre cell} are still intersections of half spaces (some examples are given later in Figure~\ref{fig: slanted dist allocation plot}). Furthermore, the
allocation policy can be interpreted as a greedy policy based on the
adjusted utility given by \eqref{eq: dual g with envy}, which contains additional interaction terms that take envy into account. 






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Old "normal partition based" solution structure %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
We now define a specific form of partition that we call the \emph{normal
partition}.
\begin{definition}
An $n$-dimensional normal partition is an $n$-partition of the probability
space $\{\Omega_1,\ldots, \Omega_n\}$ characterized by a ``shift
vector'' $v\in \bbR^n$:
$$\Omega_i
=\left\{X \in \bbR^n: i = \min \left( \argmax_j (X + v)_j\right)\right\}$$
\end{definition}
The minimum used in the definition is there to break the ties in cases where
multiple recipients have the same exact $X_i + v_i$ values. We focus on continuous
distributions in this paper, which means that the cases that require
tie-breaking have measure zero.
Ignoring these cases, $X$ is matched to $i$ if:
$$X_i + v_i > X_j + v_j \qquad \forall j\neq i$$
Geometrically, the boundaries of a normal partition consist of orthogonal
hyperplanes that all intersect at the line that goes through $-v$ and with
direction $[1,1,\ldots, 1]$.
We note here that since some regions of the space might contain zero probability
measure, multiple normal partitions could give rise to the same
matching policy for a given distribution. However, as we show later in
Lemma~\ref{lem:unique normal partition}, the normal partition for a given
matching distribution is unique up to measure-zero differences. Given this
definition for normal partitions, we now describe our main algorithmic idea. 

\begin{algorithm}
    \DontPrintSemicolon % Some LaTeX compilers require you to use \dontprintsemicolon instead
    \KwIn{Distribution $\cD$, and target matching distribution $\optp$.}
    Find the unique Normal Partition $\{\Omega_i\}$ for $\cD$ that satisfies the
    target matching distribution $\optp$.\;
    For each donor $X$, match it according to $\{\Omega_i\}$, i.e., match $X$ to
    $i$ if $X\in \Omega_i$.\;
    \caption{Normal Partition Matching}
    \label{algo: Normal Partition Matching}
\end{algorithm}

To show that Algorithm~\ref{algo: Normal Partition Matching} is optimal, we need
the following two intermediate lemmas.  We prove them under the following
regularity assumption. 
\begin{assumption}
    \label{assumption: regularity of the distribution}
    Assume that the support of distribution of
    values is bounded, i.e., $X_i \in [0, \bar x]$. Also assume that the probability
    density function is bounded, i.e. for any direction $w$, and any $\epsilon>0$, 
    $$P(\{X : w^\top X\leq c+\epsilon \}) - P(\{X : w^\top
    X\leq c \})\leq \epsilon \bar\mu$$ 
\end{assumption}
The boundedness condition ensures that we can find a shift vector $v$ within
some bounded region.  The second condition ensures that the matching
probabilities cannot change too much when the shift vector is perturbed by a
little bit.  These two assumptions are analogous to assuming bounded diameter of
the constraint set, and bounded gradients for the objective functions, both of
which are standard assumptions in optimization.
% \begin{figure*}[]
%     \begin{minipage}{.5\textwidth}
%         \centering
%         \includegraphics[width=.6\linewidth]{offset headon view.png}
%         \caption{Partition of the space viewed from the angle of $[1,1,1]$.}
%         \label{fig:partition 3D headon}
%     \end{minipage}%
%     \begin{minipage}{.5\textwidth}
%         \centering
%         \includegraphics[width=.6\linewidth]{offset offset view.png}
%         \caption{Partition of the space viewed from an offset angle.}
%         \label{fig:partition 3D offset}
%     \end{minipage}
%     \caption{An example of of partition of the probability space in 3D. In this case, $p_A =? $ (Blue axis), $p_B = ?$ (red axis), $p_C =? $ (green axis). }
%     \label{fig:partition 3D}
% \end{figure*}




\begin{lemma}
    Given any normal partition (characterized by shift vector $v$), and
    probability measure $P$ over $\bbR^n$ satisfying Assumption~\ref{assumption:
    regularity of the distribution}, suppose the resulting matching distribution
    is $[\optp_1,\ldots, \optp_n]$, i.e., $P(\Omega_i)=\optp_i$. Then this normal partition
    is a solution to \eqref{prob: optimal partition problem}.
    %  for this target
    % matching distribution $\optp = p$. 
    Moreover, for any other partition
    $\{\tilde\Omega_i\}$ such that $\bbP(\tilde\Omega_i)=\optp_i\,\forall i$, and where 
    there exists $i$ such that $\bbP(\Omega_i \cap \tilde\Omega_i)\neq \optp_i$, 
    the normal partition $\{\Omega_i\}$ has a strictly higher objective than
    $\{\tilde\Omega_i\}$.
    \label{lem: normal partition is optimal}
\end{lemma}
\begin{proof}
Given a normal partition with shift vector $v$ (and the corresponding partition
representation $\{\Omega_i\}$), the matched weights given by this normal partition
is 
\begin{align}
&\sum_i\int_{X\in\Omega_i}X_i\,dP(X) \nonumber\\
=& \int_{X\in\bbD}\max_i \left(X_i+v_i\right)\,dP(X) -
\sum_i \optp_iv_i\label{eq: normal partition matched weights}
\end{align}
The last equality holds by the definition of a normal partition, and the fact
that we know the matching distribution is $[\optp_1,\ldots, \optp_n]$.
    
Consider an alternative partition (not necessarily a normal partition) $\{\tilde
\Omega_i\}$ that has the same matching distribution, and its' corresponding
matching policy $\tilde\pi$.  The matched weights for this partition is (here we
abuse the notation for matching policy $\pi(X)$ to also mean the index that
$X$ is matched to):
\begin{align}
&\sum_i\int_{X\in\tilde \Omega_i}X_i\,dP(X) \nonumber\\
=&\sum_i\int_{X\in\tilde\Omega_i} X_i+v_i\,dP(X) - \sum_i \optp_iv_i\nonumber\\
=&\int_{X\in\bbD} X_{\tilde \pi(X)}+v_{\tilde \pi(X)}\,dP(X) - \sum_i \optp_iv_i\label{eq: alternative matched weights}
\end{align}
Again the first equality follows because we know that recipient $i$ is matched
exactly $\optp_i$ fraction of the times. Comparing \eqref{eq: normal partition
matched weights} with \eqref{eq: alternative matched weights}, it is clear that
\eqref{eq: normal partition matched weights}$\geq$\eqref{eq: alternative matched
weights}.  So the normal partition is optimal. Additionally, if there exists $i$
such that $P(\Omega_i\cap \tilde\Omega_i) < p_i$, then the normal partition has
strictly better matched weights. This is because we assume continuous distribution:
$$P\left(\bigcup\limits_{i<j}\{X: X_i +v_i= X_j+v_j\}\right) = 0$$
Therefore $P(\Omega_i\cap \tilde\Omega_i) < p_i$ implies that $$P\left(\max_i
(X_i+v_i) > X_{\tilde\pi(X)} + v_{\tilde\pi(X)}\right)
>0,$$ and so \eqref{eq: normal partition matched weights}$>$\eqref{eq:
alternative matched weights}.
    
\end{proof}

\begin{lemma}
    Given any probability measure $P$ over $\bbR^n$ satisfying
    Assumption~\ref{assumption: regularity of the distribution}, and any target
    matching distribution $[\optp_1, \ldots, \optp_n]$, there exists a
    unique\footnote{Unique up to differences with measure zero.} normal partition
    such that the partition for each recipient has measure $\optp_i$. 
    \label{lem:unique normal partition}
\end{lemma}

The proof of Lemma~\ref{lem:unique normal partition} is constructive, and relies
on an algorithm presented in a later section. So we defer the proof of
Lemma~\ref{lem:unique normal partition} to Section~\ref{sec: computing the
solution}.
    
\begin{theorem}
Algorithm~\ref{algo: Normal Partition Matching} is optimal for any target matching distribution
and any probability distribution $\cD$ satisfying Assumption~\ref{assumption:
regularity of the distribution}.
\label{thm:optimal partition}
\end{theorem}
\begin{proof}
    Lemma~\ref{lem:unique normal partition} implies that the algorithm is well
    defined, and Lemma~\ref{lem: normal partition is optimal} shows that it is
    optimal.
\end{proof}
It is worth noting that the resulting matching policy from a normal partition is
extremely simple to implement: one simply adds the shift vector to the vector of
values for each item, and match it to the recipient who has the highest adjusted
value. In addition, it is also interpretable and simple to explain (there are only
$n$ parameters, each associated with one recipient), which can be valuable in
practice. 
% In the next subsection, we prove Lemma~\ref{lem: normal partition is optimal}.
\fi




==> NeurIPS 22/StochasticOptimization.tex <==
In Section~\ref{sec: solution structure} we showed that the optimal allocation policy to our problem has a simple geometric structure in the form of Laguerre cells. In this section we present a practical algorithm for actually computing the optimal Laguerre cells. First we show that
the objective function $\cE(g, \gamma)$ in \eqref{prob: optimal matching policy problem}
is concave by rewriting the objective as follows:
\begin{equation}
    \label{eq: dual objective integration version}
    \cE(g, \gamma) = \int_{\cX} \min_{i\in [n]} \dualg(x, y_i) d\alpha(x) + g^\top \beta - \sum_{j,k, j\neq k}\gamma_{jk}\lambda_j
\end{equation}
Since $\dualg(x, y_j)$ is linear in $g$ and $\gamma$ and taking a minimum preserves concavity, the objective function is
concave. 
Therefore, the dual problem is a constrained convex optimization problem. 
The gradient of $\cE(g, \gamma)$ can be computed as follows:
\begin{align}
    \nabla_g \cE(g, \gamma)_j &= -\int_{\bbL_{y_j}(g, \gamma)} d\alpha(x) + \beta_j\label{eq: dual g gradient}\\
    \nabla_\gamma \cE(g, \gamma)_{jk} &= \int_{\bbL_{y_j}(g, \gamma)} c(x, y_j)d\alpha(x)
     - \int_{\bbL_{y_k}(g, \gamma)} c(x, y_j)\frac{\beta_j}{\beta_k}\,d\alpha(x) - \lambda_j\label{eq: dual gamma gradient}
\end{align}

\begin{algorithm}
	\DontPrintSemicolon % Some LaTeX compilers require you to use \dontprintsemicolon instead
	\KwIn{Distribution $\alpha$, target matching distribution $\optp$, timesteps $T$.}
	Initialize $g_0 = 0, \gamma_0 = 0, \eta = \frac{1}{\sqrt{T}}$.\;
	\For{$t \gets 0, 1, 2, \ldots, T$} {
	    Sample $x_t \sim \alpha$\;
	    $g_{t+1} \leftarrow g_t + \eta  \hat\nabla_g \cE(g, \gamma)$\;
	    $\gamma_{t+1} \leftarrow \left(\gamma_{t} + \eta \hat\nabla_\gamma \cE(g, \gamma)\right)^+$\;
	}
	\KwRet{$\sum_{t=1}^T g_t/T, \sum_{t=1}^T \gamma_t/T$}
	\caption{Projected SGD for Envy Constrained Optimal Transport}
	\label{algo: Projected SGD for Envy Constrained Optimal Transport}
    \end{algorithm}
Calculating this gradient is hard, as it involves integration over an arbitrary
measure $\alpha$. However, an unbiased, stochastic version of the gradient can
be easily obtained from a single sample $x\sim \alpha$:
\begin{align}
    \hat\nabla_g \cE(g, \gamma)_j &= -\1[x \in \bbL_{y_j}(g, \gamma)] + \beta_j\label{eq: dual g gradient stochastic}\\
    \hat\nabla_\gamma \cE(g, \gamma)_{jk} &=  c(x, y_j)\1[x \in \bbL_{y_j}(g, \gamma)]
    - c(x, y_j)\frac{\beta_j}{\beta_k}\1[x \in \bbL_{y_k}(g, \gamma)]- \lambda_j\label{eq: dual gamma gradient stochastic}
\end{align}
The details of the algorithm is given in Algorithm~\ref{algo: Projected SGD for
Envy Constrained Optimal Transport}.  Standard projected SGD analysis (see for
example \cite{harvey2018machine}) tells us that Algorithm~\ref{algo: Projected
SGD for Envy Constrained Optimal Transport} converges at the rate
$\cE(g^*, \gamma^*)-\cE\left(\bbE[g_T], \bbE[\gamma_T]\right)\leq
O\left(\frac{1}{\sqrt{T}}\right)$.





==> NeurIPS 22/preamble.tex <==
% %% Sets page size and margins
% % \usepackage[a4paper,top=1in,bottom=1in,left=1in,right=1in]{geometry}

% %% Paragraph styles
% %\newlength{\oldparindent}
% %\setlength{\oldparindent}{\parindent}
% %\newcommand{\myindent}{\hspace{\oldparindent}}
% %\setlength{\parindent}{0pt}

% %% Useful packages
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{mathtools} % for the defined as := sign
\usepackage{bbm} % For indicator function alikes, \mathbbm{1}
\usepackage{bm} % For bold face in math mode \bm{\omega}
\usepackage{graphicx}
\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
%\usepackage[colorlinks=true, allcolors=blue]{hyperref}
%\usepackage{cleveref} %has to be imported after hyperref
% \usepackage[colorinlistoftodos]{todonotes}



% %% New commands
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\newtheorem{claim}{Claim}
\newtheorem{definition}{Definition}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{assumption}{Assumption}

\newcommand{\sycomment}[1]{\textcolor{red}{#1}}


\newcommand{\1}{\mathbbm{1}}
\newcommand{\innerprod}[1]{\langle #1 \rangle}
%% Defining blackboard, caligraphic and bold shortcuts
\def\ddefloop#1{\ifx\ddefloop#1\else\ddef{#1}\expandafter\ddefloop\fi}
% \bbA, \bbB, ...
\def\ddef#1{\expandafter\def\csname bb#1\endcsname{\ensuremath{\mathbb{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop

% \cA, \cB, ...
\def\ddef#1{\expandafter\def\csname c#1\endcsname{\ensuremath{\mathcal{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop

% \vA, \vB, ..., \va, \vb, ...
\def\ddef#1{\expandafter\def\csname v#1\endcsname{\ensuremath{\boldsymbol{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZabcdefghijklmnopqrstuvwxyz\ddefloop

% \valpha, \vbeta, ...,  \vGamma, \vDelta, ...,
\def\ddef#1{\expandafter\def\csname v#1\endcsname{\ensuremath{\boldsymbol{\csname #1\endcsname}}}}
\ddefloop {alpha}{beta}{gamma}{delta}{epsilon}{varepsilon}{zeta}{eta}{theta}{vartheta}{iota}{kappa}{lambda}{mu}{nu}{xi}{pi}{varpi}{rho}{varrho}{sigma}{varsigma}{tau}{upsilon}{phi}{varphi}{chi}{psi}{omega}{Gamma}{Delta}{Theta}{Lambda}{Xi}{Pi}{Sigma}{varSigma}{Upsilon}{Phi}{Psi}{Omega}{ell}\ddefloop





% \usepackage[shortlabels]{enumitem} % \begin{enumerate}[(a)], or \begin{enumerate}[a)]

%% Bibliography setup
% To use a different bibliography style, just change "numeric" to
% your preferred style (mla for MLA style, alphabetic for Author-Year
% style, etc.) There are a lot of options; check the BibLaTeX documentation.
\usepackage[backend=bibtex,style=numeric]{biblatex}
% Select the bibliography file
\addbibresource{sources.bib}

